Optimal Reads-From Consistency Checking for C11-Style Memory Models

Over the years, several memory models have been proposed to capture the subtle concurrency semantics of C/C++.One of the most fundamental problems associated with a memory model M is consistency checking: given an execution X, is X consistent with M? This problem lies at the heart of numerous applications, including specification testing and litmus tests, stateless model checking, and dynamic analyses. As such, it has been explored extensively and its complexity is well-understood for traditional models like SC and TSO. However, less is known for the numerous model variants of C/C++, for which the problem becomes challenging due to the intricacies of their concurrency primitives. In this work we study the problem of consistency checking for popular variants of the C11 memory model, in particular, the RC20 model, its release-acquire (RA) fragment, the strong and weak variants of RA (SRA and WRA), as well as the Relaxed fragment of RC20. Motivated by applications in testing and model checking, we focus on reads-from consistency checking. The input is an execution X specifying a set of events, their program order and their reads-from relation, and the task is to decide the existence of a modification order on the writes of X that makes X consistent in a memory model. We draw a rich complexity landscape for this problem; our results include (i)~nearly-linear-time algorithms for certain variants, which improve over prior results, (ii)~fine-grained optimality results, as well as (iii)~matching upper and lower bounds (NP-hardness) for other variants. To our knowledge, this is the first work to characterize the complexity of consistency checking for C11 memory models. We have implemented our algorithms inside the TruSt model checker and the C11Tester testing tool. Experiments on standard benchmarks show that our new algorithms improve consistency checking, often by a significant margin.

==> algorithms/algo-HB.tex <==
%!TEX root=../main.tex

\begin{algorithm*}[t]
\myfun{\getHBTS{$\E$, $\po$, $\rf$}}{
    \ForEach{$t, t' \in E.tids$}{ \label{line:hb-clock-init}
        $\Hh_{t}[t'] \gets 0$; 
        $\LRFH_t[t'] \gets 0$;
        $\SW_{t}[t'] \gets 0$
    }
    $\HB \gets []$;
    $\Uu \gets []$;
    $\LRFArr \gets []$ \;
    \ForEach{$\event \in \E$ in $(\po \cup \rf)$-order}{
        \Let $t = \event.\tid$ \;
        $\Hh_{t}[t] \gets \Hh_{t}[t] + 1$ \;
        \Case{$\event = \rd(t, x)$}{
            \Let $w = \rf(\event)$ \label{line:hb-read-start} \;
            \Let $T_w$ = \lIf*{$w.\ord \sqsupseteq \MOrel$}{$\HB[w]$} \lElse*{$\LRFArr[w]$} \;
            \tcp{Update $\Hh_t$}
            \If{$\event.\ord \sqsupseteq \MOacq$}{
                % $\Hh_t \gets \Hh_t \mx \LRFArr[w]$ \tcp{$\mx$ stands for point-wise maximum} \label{line:HB-read-LRFArr}
                $\Hh_t \gets \Hh_t \mx T_w$ \tcp{$\mx$ stands for point-wise maximum} \label{line:HB-read-LRFArr}
                \lIf{$w.\op = \ud$}{$\Hh_t \gets \Hh_t \mx \Uu[w]$ \label{line:HB-read-RMW}}
            }
            \tcp{Update $\SW_t$}
            % $\SW_t \gets \SW_t \mx \LRFArr[w]$ \label{line:HB-read-LRFArr-SW} \;
            $\SW_t \gets \SW_t \mx T_w$ \label{line:HB-read-LRFArr-SW} \;
            \lIf{$w.\op = \ud$}{ 
                $\SW_t \gets \SW_t \mx \Uu[w]$ \label{line:hb-read-end}
            }
        }
        \Case{$\event = \wt(t, x)$}{
            \tcp{Update $\LRFArr$}
            % \lIf{$\event.\ord \sqsupseteq \MOrel$}{
            %     $\LRFH_t \gets \Hh_t$ \label{line:hb-write-start}
            % }
            $\LRFArr[\event] \gets \LRFH_t$ \label{line:hb-write-end}

        }
        \Case{$\event = \ud(t, x)$}{
            Execute \cref{line:hb-read-start}--\cref{line:hb-read-end} and \cref{line:hb-write-end} \;
            \tcp{Update $\Uu$}
            % $\Uu[\event] \gets \LRFArr[w]$ \;
            $\Uu[\event] \gets T_w$ \;
            % $\Uu[\event] \gets$ \lIf*{$w.\ord \sqsupseteq \MOrel$}{$\HB[w]$} \lElse*{$\LRFArr[w]$} \;
            \lIf{$w.\op = \ud$}{
                $\Uu[\event] \gets \Uu[\event] \mx \Uu[w]$
            }
            % \tcp{Update $\LRFArr$}
            % $\LRFArr[\event] \gets \LRFH_t$
        }
        \Case{$\event = \fnc$}{
            \tcp{Update $\Hh_t$}
            \lIf{$\event.\ord \sqsupseteq \MOacq$}{
                $\Hh_t \gets \Hh_t \mx \SW_t$
            }
            % \tcp{Update $\LRFH_t$ and $\LRFArr$}
            \tcp{Update $\LRFH_t$}
            \lIf{$\event.\ord \sqsupseteq \MOrel$}{
                $\LRFH_t \gets \Hh_t$
                % $\LRFArr[\event] \gets \LRFH_t$
            }
        }
        $\HB[e] \gets \Hh_t$
    }
    \Return $\HB$  
}
\caption{\textit{Computing $\hb$-timestamps.}}
\label{algo:hb-timestamps}
\end{algorithm*}


==> algorithms/algo-lastWrite-old.tex <==
%!TEX root = main.tex

\begin{algorithm*}[t]
\myfun{\getLRWB{$\E$, $\po$}}{
    \lForEach{$t \in \E.tids$}{
       $n_t \gets 0$
    }
    \lForEach{$t \in \E.tids, x \in \E.locs$}{
       % $\event_{\rd, t, x}, \event_{\wt, t, x} \gets \nil, \nil$
        $\event_{\rd, t, x}, \event_{\wt, t, x} \gets \bot, \bot$
    } 
    $\LRB, \LWB \gets [], []$ \;
    \ForEach{$\event \in \E$ in $\po$-order}{
        \Let $t = \event.\tid$, $x = \event.\lloc$ \;
        $n_t \gets n_t + 1$ \;
        \lIf{$\event.\op \in \set{\rd, \ud}$}{
             $\event_{\rd, t, x} \gets \event$
        }
        \lIf{$\event.\op \in \set{\wt, \ud}$}{
             $\event_{\wt, t, x} \gets \event$
        }
        \lForEach{$y \in \E.locs$}{
            $\LRB[t][y][n_t], \, \LWB[t][y][n_t] \gets \event_{\rd, t, y}, \, \event_{\wt, t, y}$
        }
    }
    \Return ($\LRB$, $\LWB$)  
}
\BlankLine
\myfun{\getLRB{$\E$, $\po$}}{
    $(\LRB,\LWB) \gets$ \getLRWB{$\E$, $\po$} \;
    \Return $\LRB$
}
\BlankLine
\myfun{\getLWB{$\E$, $\po$}}{
    $(\LRB,\LWB) \gets$ \getLRWB{$\E$, $\po$} \;
    \Return $\LWB$
}
\caption{\label{algo:last-write-before}
Computing the functions $\glw(t, x, i)$ and $\glr(t, x, i)$.
}
\end{algorithm*}
\normalsize


==> algorithms/algo-lastWrite.tex <==
%!TEX root = ../main.tex

\begin{algorithm*}[t]
\ForEach{$t, u \in \E.tids, x \in \E.locs$}{
    $\view{\WtLst}{t,x}{u}, \view{\RdLst}{t,x}{u} \gets \emptyset, \emptyset$ \;
    $\view{\wt\mathtt{ptr}}{t,x}{u}, \view{\rd\mathtt{ptr}}{t,x}{u} \gets \bot, \bot$
}
\BlankLine
\myfun{\initWtRdLst{$\E$, $\po$}}{
    \lForEach{$t \in \E.tids$}{
       $n_t \gets 0$
    } 
    \ForEach{$\event \in \E$ in $\po$-order}{
        \Let $t = \event.\tid$, $x = \event.\lloc$ \;
        $n_t \gets n_t + 1$ \;
        \If{$\event.\op \in \set{\rd, \ud}$}{
            \lForEach{$u \in \E.tids$}{
            $\insLst{\view{\WtLst}{t,x}{u}}{$\langle n_t,\event\rangle$}$
            }
        }
        \If{$\event.\op \in \set{\wt, \ud}$}{
             \lForEach{$u \in \E.tids$}{
                $\insLst{\view{\RdLst}{t,x}{u}}{$\langle n_t,\event\rangle$}$
            }
        }
    }
    \ForEach{$t, u \in \E.tids, x \in \E.locs$}{
        $\view{\wt\mathtt{ptr}}{t,x}{u} \gets \first{\view{\WtLst}{t,x}{u}}$ \;
        $\view{\rd\mathtt{ptr}}{t,x}{u} \gets \first{\view{\RdLst}{t,x}{u}}$
    }
    \Return ($\set{\view{\WtLst}{t,x}{u}}_{t, x, u}$, $\set{\view{\RdLst}{t,x}{u}}_{t, x, u}$)  
}
\BlankLine
\myfun{\initWtLst{$\E$, $\po$}}{
    $(\set{\view{\WtLst}{t,x}{u}}_{t, x, u},\set{\view{\RdLst}{t,x}{u}}_{t, x, u}) \gets$ \initWtRdLst{$\E$, $\po$} \;
    \Return $\set{\view{\WtLst}{t,x}{u}}_{t, x, u}$
}
\BlankLine
\myfun{\initRdLst{$\E$, $\po$}}{
    $(\set{\view{\WtLst}{t,x}{u}}_{t, x, u},\set{\view{\RdLst}{t,x}{u}}_{t, x, u}) \gets$ \initWtRdLst{$\E$, $\po$} \;
    \Return $\set{\view{\RdLst}{t,x}{u}}_{t, x, u}$
}
\BlankLine
\myfun{$\apicall{\view{\WtLst}{t,x}{u}}{get}{c}$}{
    % $\langle n_t, \event \rangle \gets \view{\wt\mathtt{ptr}}{t,x}{u}$ \;
    $\wt \gets \bot$ \;
    \While{$\view{\wt\mathtt{ptr}}{t,x}{u} \neq \listLast{\view{\WtLst}{t,x}{u}}$}{
        $\langle n_t, \event \rangle \gets \view{\wt\mathtt{ptr}}{t,x}{u}$ \;
        \lIf{$n_t > c$}{\Break}
        $\wt \gets \event$ \;
        $\view{\wt\mathtt{ptr}}{t,x}{u} \gets \listNext{\view{\WtLst}{t,x}{u}}$
    }
    \Return $\wt$
}
\BlankLine
\myfun{$\apicall{\view{\RdLst}{t,x}{u}}{get}{c}$}{
    % $\langle n_t, \event \rangle \gets \view{\wt\mathtt{ptr}}{t,x}{u}$ \;
    $\rd \gets \bot$ \;
    \While{$\view{\rd\mathtt{ptr}}{t,x}{u} \neq \listLast{\view{\RdLst}{t,x}{u}}$}{
        $\langle n_t, \event \rangle \gets \view{\rd\mathtt{ptr}}{t,x}{u}$ \;
        \lIf{$n_t > c$}{\Break}
        $\rd \gets \event$ \;
        $\view{\rd\mathtt{ptr}}{t,x}{u} \gets \listNext{\view{\RdLst}{t,x}{u}}$
    }
    \Return $\rd$
}

\caption{\label{algo:last-write-before}
Data structure for computing $\glw(t, x, i)$ and $\glr(t, x, i)$.
}
\end{algorithm*}
\normalsize


==> algorithms/algo-ra-rf-on-the-fly-helper.tex <==
%!TEX root = main.tex

	
	\begin{algorithm*}[t]
		%\Input{Events $\E$, program order $\po$ and reads-from relation $\rf$, }
		\BlankLine
		
		
		
		\BlankLine
		\myfun{\getLW{$t, x, timestamp$}}{
			\Let $\E = $ Events s.t. $e.\op =\wt \lor \ud$, $e.\tid = t$, $e.\lloc = x$ and $\HB[e][t] \leq timestamp$ \;
			\Let $w = $ Last executed event in $\E$ \;
			\Return $w$
		}
		
		\BlankLine
		\myfun{\poprop{$w$}}{
			\Let $\E = $ Events that are $\po$ ordered after $w$ \;
			\ForEach{$e \in \E$}{
				$\HBMO[e] \gets \HBMO[e] \mx \HBMO[w]$
			}
		}
		
		\BlankLine
		\myfun{\joinchangedindex{clock1, clock2}}{
			$clock1'$ = $clock1$ \;
			$clock1 = clock1 \mx clock2$ \;
			\ForEach{$t \in tids$}{
				\If {$clock1[t] \neq clock1'[t]$} {
					$clock1.\mathsf{changedIndexes.\mathsf{add}(t)}$
				}
			}
			\Return $clock1$
		}
		
		
		\caption{Helper Functions for On-The-Fly Checking of RF Consistency for RA.}
		\label{algo:ra-rf-on-the-fly-helper}
	\end{algorithm*}
	
	
	\normalsize


==> algorithms/algo-tc-pc.tex <==
%!TEX root = main.tex

\begin{algorithm*}[t]
\myfun{\getTCPC{$\E$, $\rf$}}{
    $\TC, \PC \gets [], []$ \;
    \ForEach{$\event \in \E$ in $\rf$-order}{
        \lIf{$\event.\op = \wt$}{
            $\TC[\event] \gets \event$; 
            $\PC[\event] \gets 0$
        }
        \lIf{$\event.\op = \ud$}{
            $\TC[\event] \gets \TC[\rf(\event)]$; 
            $\PC[\event] \gets \PC[\rf(\event)] + 1$
        }
    }
    \Return ($\TC$, $\PC$)  
}
\caption{Computing the functions $\TC$ and $\PC$.}
\label{algo:tc-pc}
\end{algorithm*}
\normalsize


==> app_hb.tex <==
\subsection{Proof of {\cref{lem:HB-computation}}}\label{subsec:app_proof_hb_computation}

\newcommand{\lst}{\mathsf{last}}
\newcommand{\lsti}[1]{{(#1),\lst}}
\newcommand{\relfence}{\fnc,\MOrel}
\newcommand{\locIdx}{\mathsf{locIdx}}


\input{algorithms/algo-HB}

We state the detailed invariants maintained by \cref{algo:hb-timestamps} in \cref{lem:hb-invariant}.
These invariants can be established using induction.
Further, \cref{lem:HB-computation} follows as a corollary of \cref{lem:hb-invariant}.

For an event $e$ of thread $t$, we use the notation
$\locIdx(e) = |\setpred{f}{(f, e) \in \po^?}|$ to denote the position of $e$ within its own thread.
It follows that $\HB_e(u) = \max\setpred{\locIdx(f)}{(f, e) \in \hb^?}$.
For a sequence $\sigma$ of events, we use $\lst(\sigma, \E)$ to denote the last
event in $\sigma$ which belongs to $\E$. 
For example, $\lst(\sigma, \F_{\sqsupseteq \MOrel}^{t})$ to denote the last event $e \in \sigma$
such that $e.\tid = t$, $e.\op = \fnc$ and $e.\ord \in \set{\MOrel, \MOacqrel}$.

\begin{restatable}{lemma}{HB-invariant}\label{lem:hb-invariant}
Let $\E$, $\po$ and $\rf$ be inputs to  \cref{algo:hb-timestamps} 
such that $(\po \cup \rf)$ is acyclic.
Let $\pi = e_1, e_2 \ldots, e_n$ 
be the sequence in which \cref{algo:hb-timestamps} processes events from $\E$.
Let $i \geq 0$, let $\pi_i = e_1, \ldots, e_i$ be the prefix of $\pi$ of length $i$ (with $\pi_0 = \epsilon$).
% For a thread $t$, 
% let $e^\lsti{i}_t$ denote the last event $e$ in $\pi_i$ for which $e.\tid = t$.
% and let $e^{\lsti{i}}_{t, \relfence}$ be the
% last event $e$ in $\pi_i$ for which $e.\tid = t$, $e.\op = \fnc$ and $e.\ord = \MOrel$.
Further, let $\Hh_t^{(i)}$, $\LRFH_t^{(i)}$, $\SW_t^{(i)}$, $\Uu^{(i)}$,
$\HB^{(i)}$ and $\LRFArr^{(i)}$ be the values of 
respectively $\Hh_t$, $\LRFH_t$, $\SW_t$, $\Uu$,
$\HB$ and $\LRFArr$ 
after having processed the prefix $\pi_i$. 
Then, we have the following.
\begin{enumerate} 
	\item\label{item:HB-Hh} $\Hh_t^{(i)} = \HB_e$, where $e = \lst(\pi_i, \E^t)$. 
	If no such $e$ exists in $\pi_i$, then $\Hh_t^{(i)} = \lambda u, 0$.
	\item\label{item:HB-HB} For an $e \in \pi_i$, $\HB^{(i)}[e] = \HB_e$. 
	% \item\itmlabel{HB-LRFH} $\LRFH_t^{(i)} = \HB_e$, where $e = \lst(\pi_i, \F_{\sqsupseteq \MOrel}^{t})$.
	\item\label{item:HB-LRFH} 
	\[
	\LRFH_t^{(i)} = 
	\begin{cases}
		\HB_e & \text{ if } e = \lst(\pi_i, \E^t) \text{ exists}, e.\op \in \set{\wt, \ud} \text{ and } e.\ord \sqsupseteq \MOrel \\
		\HB_e & \text{ otherwise, if } e =  \lst(\pi_i, \F_{\sqsupseteq \MOrel}^{t}) \text{ exists} \\
		\lambda u, 0 & \text{ otherwise}
	\end{cases}
	\]
	% $\LRFH_t^{(i)} = \HB_e$, 
	% with $e = \lst(\pi_i, \F_{\sqsupseteq \MOrel}^{t} \cup S)$,
	% where $S = \set{\lst(\pi_i, \E^t)}$ if $\lst(\pi_i, \E^t).\op \in \set{\wt, \ud}$ and $\lst(\pi_i, \E^t).\ord \sqsupseteq \MOrel$,
	% and $S = \emptyset$ otherwise.
	% If no such $e$ exists, then $\LRFH_t^{(i)} = \lambda u, 0$.
	\item\label{item:HB-LRFArr} For an $e \in \pi_i$,
	 such that $e.\op \in \set{\wt, \ud}$, 
	% $\LRFArr^{(i)}[e] = \HB_f$, where $f$ 
	% is the last event in $\pi_i$ for which $f.\op \in \set{\fnc, \wt, \ud}$, $f.\tid = e.\tid$, $f.\ord \sqsupseteq \MOrel$ and  $(f, e) \in \po^?$.
	% If no such $f$ exists, or if $e.\op \not\in \set{\wt, \ud}$ then $\LRFArr^{(i)}[e]$ is undefiend.
	\[
	\LRFArr^{(i)}[e] = 
	\begin{cases}
		\HB_e & \text{ if } e.\ord \sqsupseteq \MOrel \\
		\HB_f & 
		\text{ otherwise if } 
		\begin{array}{c}
		f \text{ is the last event with } \\
		(f, e) \in \po, f.\op = \fnc, f.\ord \sqsupseteq \MOrel
		\end{array} \\
		\lambda u, 0 & \text{ otherwise if no such $f$ exists}
	\end{cases}
	\]
	If $e.\op \not\in \set{\wt, \ud}$ then $\LRFArr^{(i)}[e]$ is undefiend
	\item\label{item:HB-SW} $\SW_t^{(i)}[u] = \locIdx(e)$, where $e$ is the last event in $\pi_i$
	such that $e.\tid = u$ and $(e, \lst(\pi_i, \E^t)) \in \hb^?;[\E_{\sqsupseteq \MOrel}];([\F];\po)^?;\rf^+;\po^?$.
	If no such $e$ exists, then $\SW_t^{(i)}[u] = 0$. \\
	Observe that since $\pi_i$ is consistent with $\hb \subseteq (\po \cup \rf)^+$,
	if $e$ exists in $\pi$, then it exists in $\pi_i$ too.
	\item\label{item:HB-RMW} For an event $e \in \pi_i$ such that $e.\op = \ud$,
	$\Uu^{(i)}[e][t] = \locIdx(f)$, where $f$ is the last event in $\pi$
	such that $f.\tid = t$ and $(f, e) \in \hb^?;[\E_{\sqsupseteq \MOrel}];([\F];\po)^?;\rf^+$ --- notice that
	we require that the path from $f$ to $e$ ends in an $\rf$ edge and not a $\po$ edge.
	If no such $f$ exists, then $\Uu^{(i)}[e][t] = 0$. \\
	As before, since $\pi_i$ is consistent with $\hb \subseteq (\po \cup \rf)^+$,
	if $e$ exists in $\pi$, then it exists in $\pi_i$ too. \\
	If $e.\op \neq \ud$ then $\Uu^{(i)}[e]$ is undefiend
\end{enumerate}
\end{restatable}

\begin{proof}
We prove this by induction on the length $i$ of the prefix processed by the algorithm.
In the base case $(i = 0)$, the invariants \cref{item:HB-HB}, \cref{item:HB-LRFArr} and \cref{item:HB-RMW} vacuously hold as there in no $e \in \pi_i$. The other three invariants also hold because the corresponding clocks $\Hh_t$, $\LRFH_t$ and $\SW_t$ are initialized with $\lambda u, 0$.

Let us consider the inductive case. Assume that all the invariants
 \cref{item:HB-Hh}, \cref{item:HB-HB}, \cref{item:HB-LRFH}, \cref{item:HB-LRFArr}, 
 \cref{item:HB-SW} and \cref{item:HB-RMW} hold for the prefix $\pi_i = e_1, e_2, \ldots, e_i$, 
 and argue why they will hold for length $\pi_{i+1} = \pi_i e_{i+1}$.
Let $t = e_{i+1}.\tid$.
First let us argue that the timestamps corresponding to all 
previous events remain unchanged in the new prefix $\pi_{i+1}$.
First, the $\HB$-timestamp of an event $e$ only depend upon events that are $(\po\cup\rf)^+$-before $e$
and thus must precede $e$ in $\pi_{i+1}$.
Likewise, $\LRFArr[e] = f$ implies that $f$ must be $\po^?$-before $e$ and thus must appear prior to $e$ in $\pi_{i+1}$.
Similarly, $\Uu^{(i)}[e][t] = \locIdx(f)$ implies that $f$ is $(\po\cup\rf)^+$-before $e$ and thus must appear prior to $e$ in $\pi_{i+1}$.
We can similarly argue that the value of all clocks associated with a thread $u \neq t$ must remain unchanged
because they record information about some event of the form $e = \lst(\pi_i, \E^u)$ or $e = \lst(\pi_i, \F_{\sqsupseteq \MOrel}^{u})$, and events that are  $(\po\cup\rf)^+$-before $e$. Since $e$ appears in $\pi_i$ (because $u \neq e_{i+1}.\tid$), it must be that all these clocks remain unchanged.
Thus, we only need to argue about the entries corresponding to $e_{i+1}$
and how the clocks with subscript $t$ change.

We will do a case-by-case analysis based on $e_{i+1}.\op$.
Let us establish some notations and properties first.

For a $j$, let us define the set
$\E_{u, \SW_t, j} = \setpred{e \in \pi_j}{e.\tid = u, 
(e, \lst(\pi_j, \E^t)) \in \hb^?;[\E_{\sqsupseteq \MOrel}];([\F];\po)^?;\rf^+;\po^?}$.
Observe that since events of a given thread (and thus the thread $t$ in particular) are $\po$-ordered,
we have $\E_{u, \SW_t, j} \subseteq \E_{u, \SW_t, k}$ if $j \leq k$.
Thus, $\E_{u, \SW_t, i} \subseteq \E_{u, \SW_t, i+1}$.
Let us now establish the following equation
\begin{equation}
\label{eq:SW_t_induction}
\E_{u, \SW_t, i+1} = \E_{u, \SW_t, i} \cup S_{\mathsf{rf}}(e_{i+1}) \cup S_{\rf^+}(e_{i+1})
\end{equation}
where
\[
\begin{array}{rcl}
S_\rf(e) &=& \setpred{f}{e.\op \in \set{\rd, \ud}, f.\tid = u, (f, \rf(e)) \in  \hb^?;[\E_{\sqsupseteq \MOrel}];([\F];\po)^?} \\
S_{\rf^+}(e) &=& \setpred{f}{e.\op = \ud, f.\tid = u, \rf(e).\op = \ud, (f, \rf(e)) \in  \hb^?;[\E_{\sqsupseteq \MOrel}];([\F];\po)^?;\rf^+}
\end{array}
\]
First observe that $\E_{u, \SW_t, i} \subseteq \E_{u, \SW_t, i+1}$, 
$S_{\mathsf{rf}}(e_{i+1}) \subseteq \E_{u, \SW_t, i+1}$ and 
$S_{\rf^+}(e_{i+1}) \subseteq \E_{u, \SW_t, i+1}$ and thus we need to only establish that
$\E_{u, \SW_t, i+1} \subseteq \E_{u, \SW_t, i} \cup S_{\mathsf{rf}}(e_{i+1}) \cup S_{\rf^+}(e_{i+1})$.
This follows using a simple case by case analysis on how the path 
$(e, e_{i+1})$ ends for a given $e \in  \E_{u, \SW_t, i+1}$.
If it ends in a $\po$ edge, then $e \in \E_{u, \SW_t, i}$.
If it ends in a single $\rf$ edge, then $e \in S_{\mathsf{rf}}(e_{i+1})$, and finally if it ends in a sequence of $\rf$ edges,
then $e \in S_{\rf^+}(e_{i+1})$.

\newcommand{\HBBef}{\textsf{HBBef}}
Now, for an event $e$, let $\HBBef(e) = \setpred{f}{(f, e) \in \hb^?}$.
If $e$ does not exist, then we let $\HBBef(e) = \emptyset$.
Let us establish the following equation:
\begin{equation}
\label{eq:HB_induction}
\HBBef(e_{i+1}) = 
\set{e_{i+1}} \cup \HBBef(e^{\po}_{i+1}) \cup S_{\MOacq, \rd}(e_{i+1}) \cup  S_{\MOacq, \fnc}(e_{i+1})
\end{equation},
where
$e^\po_{i+1}$ is the unique event with $(e^{\po}_{i+1}, e_{i+1}) \in \po_\imm$,
\[
\begin{array}{rcl}
S_{\MOacq, \rd}(e) &=& \setpred{f}{e.\ord \sqsupseteq \MOacq, f \in S_{\mathsf{rf}}(e) \cup S_{\rf^+}(e)} \\
S_{\MOacq, \fnc}(e) &=& \setpred{f}{e.\ord \sqsupseteq \MOacq, e.\op = \fnc, \exists g, (g, e) \in \po, f \in S_{\mathsf{rf}}(g) \cup S_{\rf^+}(g)}
\end{array}
\]
The above equation follows because if $(f, e_{i+1}) \in \hb^?$, then either $f = e_{i+1}$, or
there is an event $g$ such that $(f, g) \in \hb^?$ and either (a) $(g, e_{i+1}) \in \po$, or (b) $(g, e_{i+1}) \in \sw$.
In the former case, we can take $g = e^\po_{i+1}$.
In the latter case, we have $(g, e_{i+1}) \in [\E_{\sqsupseteq \MOrel}];([\F];\po)^?;\rf^+;(\po;[\F])^?;[\E_{\sqsupseteq \MOacq]}]$ and thus $e_{i+1}.\ord \sqsupseteq \MOacq$.
If $e_{i+1}.\op \in \set{\rd, \ud}$, then it is easy to see that $f \in S_{\MOacq, \rd}(e_{i+1})$.
If on the other hand $e_{i+1}.\op = \fnc$, then it is easy to see that $f \in S_{\MOacq, \fnc}(e_{i+1})$.


\begin{description}
	\item[Case $e_{i+1}.\op = \rd$.] 
	First, observe that $\lst(\pi_i, \F_{\sqsupseteq \MOrel}^{t}) = \lst(\pi_{i+1}, \F_{\sqsupseteq \MOrel}^{t})$ and thus $\LRFH_t^{(i+1)} = \LRFH_t^{(i)}$.

	Next we consider $\SW^{(i+1)}_t[u]$ for some thread $u$.
	First, if $\SW^{(i+1)}_t[u] = 0$, then observe that
	$\E_{u, \SW_t, i+1} = 0$.
	From \cref{eq:SW_t_induction}, it follows that
	$\E_{u, \SW_t, i} = S_\rf(e_{i+1}) = \emptyset$, and further, if $w = \rf(e_{i+1})$ is an RMW, then $S_{\rf^+}(e_{i+1}) = \emptyset$.
	In this case, the updates in \cref{line:HB-read-LRFArr-SW} and \cref{line:hb-read-end}
	correctly reflect the value of $\SW^{(i+1)}_t[u]$.
	Next, we consider the case when $\SW^{(i+1)}_t[u] = m > 0$

	Let $e$ be the event such that $e.\tid = u$ and $\locIdx(e) = m = \SW^{(i+1)}_t[u]$.
	First, we observe that $e \in \E_{u, \SW_t, i+1}$ and thus
	we have one of (a) $e \in \E_{u, \SW_t, i}$, or (b) $e \in S_\rf(e_{i+1})$ or (c) $e \in S_{\rf^+}(e_{i+1})$.
	By induction we will have respectively (a) $\SW^{(i)}_t[u] \geq m$,
	(b) $\LRFArr[w][u] \geq m$, where $w = \rf(e_{i+1})$, and 
	(c) $w.\op = \ud$ with $\Uu[w][u] \geq m$.
	In each of these cases, if the inequality is strict (i.e., $> m$), then
	we know that there is another event $e'$ such that $(e, e') \in \po$ and
	one of $e' \in \E_{u, \SW_t, i}$, or $e' \in S_\rf(e_{i+1})$ or $e' \in S_{\rf^+}(e_{i+1})$ holds,
	and thus $e' \in \in \E_{u, \SW_t, i+1}$ implying that 
	$\SW^{(i+1)}_t[u] > m$ which is a contradiction.
	Thus, we have strict equality in one of (a) $\SW^{(i)}_t[u] \geq m$,
	(b) $\LRFArr[w][u] \geq m$, 
	(c) $\Uu[w][u] \geq m$.
	In this case, the updates in \cref{line:HB-read-LRFArr-SW} and \cref{line:hb-read-end}
	correctly reflect the value of $\SW^{(i+1)}_t[u]$.

	Now, we argue about $\Hh_t$.
	Here, $S_{\MOacq, \fnc}(e_{i+1}) = \emptyset$ since $e_{i+1}.\op \neq \fnc$.
	Thus, we have $\HBBef(e_{i+1}) = \set{e_{i+1}} \cup \HBBef(e^{\po}_{i+1}) \cup S_{\MOacq, \rd}(e_{i+1})$.
	As with $\SW_t$, we can argue that $\Hh_t^{(i+1)}$ is correctly updated.	


	Next, $\HB[{e_{i+1}}] = \HB_{e_{i+1}}$ follows because $e_{i+1} = \lst(\pi_{i+1}, \E^t)$.

	Finally, since $e_{i+1}.\op \neq \ud$, $\Uu[e_{i+1}]$ is undefined as also ensured by the algorithm.

	\item[Case $e_{i+1}.\op = \wt$.] 
	In this case, if $e_{i+1}.\ord \sqsupseteq \MOrel$, then we must have
	$\LRFH_t^{(i+1)} = \HB_{e_{i+1}} = \Hh^{(i+1)}_t$.
	Otherwise, $\lst(\pi_i, \F_{\sqsupseteq \MOrel}^{t}) = \lst(\pi_{i+1}, \F_{\sqsupseteq \MOrel}^{t})$ and thus $\LRFH_t^{(i+1)} = \LRFH_t^{(i)}$.
	Finally, $\LRFArr[e_{i+1}] = \LRFH_t^{(i+1)}$ as expected.

	Now, we consider $\SW^{(i+1)}_t[u]$ for some thread $u$.
	Recall $\E_{u, \SW_t, i+1} = \E_{u, \SW_t, i} \cup  S_\rf(e_{i+1}) \cup S_{\rf^+}(e_{i+1})$.
	Since $e_{i+1}.\op = \wt$, we have 
	$\E_{u, \SW_t, i+1} = \E_{u, \SW_t, i}$.
	It follows that $\SW^{(i+1)}_t[u] = \SW^{(i)}_t[u]$ and this is what the algorithm ensures.

	Finally, we consider $\Hh_t^{(i+1)}$.
	Recall that $\HBBef(e_{i+1}) = \set{e_{i+1}} \cup \HBBef(e^{\po}_{i+1}) \cup S_{\MOacq, \rd}(e_{i+1}) \cup  S_{\MOacq, \fnc}(e_{i+1})$.
	Since $e.\op \not\in \set{\rd,\ud,\fnc}$, we have 
	$\HBBef(e_{i+1}) = \set{e_{i+1}} \cup \HBBef(e^{\po}_{i+1})$ and the algorithm ensures this.

	Finally, since $e_{i+1}.\op \neq \ud$, $\Uu[e_{i+1}]$ is undefined as also ensured by the algorithm.

	\item[Case $e_{i+1}.\op = \ud$.] 
	This case follows from the above two cases, except for $\Uu[e_{i+1}]$. We will argue about $\Uu[e_{i+1}]$ next.
	Consider an event $f$ such that $(f, e_{i+1}) \in \hb^?;[\E_{\sqsupseteq \MOrel}];([\F];\po)^?;\rf^+$.
	We have two cases here. \\
	First, there is only a single trailing $\rf$ edge, i.e.,
	$(f, e_{i+1}) \in \hb^?;[\E_{\sqsupseteq \MOrel}];([\F];\po)^?;\rf$.
	In this case, $f \in S_{\mathsf{rf}}(e_{i+1})$. \\
	Otherwise, we have $(f, e_{i+1}) \in \hb^?;[\E_{\sqsupseteq \MOrel}];([\F];\po)^?;\rf^+;\rf$.
	In this case, $\rf(e_{i+1}).\op = \ud$ and further $f \in S_{\mathsf{rf}}(\rf(e_{i+1}))$.
	The correctness then follows.


	\item[Case $e_{i+1}.\op = \fnc$]
	Recall that $\HBBef(e_{i+1}) = \set{e_{i+1}} \cup \HBBef(e^{\po}_{i+1}) \cup S_{\MOacq, \rd}(e_{i+1}) \cup  S_{\MOacq, \fnc}(e_{i+1})$.
	Since $e.\op \not\in \set{\rd,\ud}$, we have 
	$\HBBef(e_{i+1}) = \set{e_{i+1}} \cup \HBBef(e^{\po}_{i+1}) \cup  S_{\MOacq, \fnc}(e_{i+1})$.
	Consider an event $e$ such that $e \in  S_{\MOacq, \fnc}(e_{i+1})$.
	This means that there is a $g$ such that $(g, e_{i+1}) \in \po$ and 
	$(e, g) \in S_\rf(g) \cup S_{\rf^+}(g)$.
	This in turn means that 
	$(e, \rf(g)) \in  \hb^?;[\E_{\sqsupseteq \MOrel}];([\F];\po)^?\rf^*$.
	Thus, $(e, e_{i+1}) \in  \hb^?;[\E_{\sqsupseteq \MOrel}];([\F];\po)^?\rf^+;\po$.
	Thus, $\SW_t^{i}[e.\tid] \geq \locIdx(e)$ by induction.

	Next, $\LRFArr[e_{i+1}]$ is undefined since $e_{i+1} \not\in \set{\wt, \ud}$.
	Finally, $\LRFH_t^{i+1} = \HB_{e_{i+1}}$ since $e_{i+1}.\op = \fnc$ and $e_{i+1} = \lst(\pi_{i+1}, \E^t)$.
\end{description}
\end{proof}

==> app_helper_functions.tex <==
%!TEX root=./main.tex

\subsection{Proofs of {\cref{sec:helper_functions}}}\label{subsec:app_helper_functions}


Here we present the algorithms for the helper functions defined in \cref{sec:helper_functions}.


\input{algorithms/algo-HB}

\bparagraph{Happens-before computation}
We start with the computation of $\hb$, performed by \cref{algo:hb-timestamps}.
As $\hb$ coincides for all models, the algorithm considers the full $\rcmm$ model that mixes release-acquire with relaxed accesses.

The algorithm works in a streaming fashion processing one event at a time,
in some order consistent with the $\po \cup \rf$ relation.
The output of the algorithm is an array $\HB$ which is indexed by events in $\E$.
To compute this array, the algorithm maintains auxiliary data structures
that capture different aspects of how the $\hb$ relation can be communicated.
At each event $\event$, the algorithm accesses the current values of these data structures,
updates some of them and computes the timestamp $\HB[\event]$.
All the data structures store either a single timestamp ($\Hh_t$, $\LRFH_t$, $\SW_t$)
or an array (indexed by events in $\E$)  
of timestamps ($\HB$, $\LRFArr$ and $\Uu$).
Informal details of the different structures used are below, while detailed invaraints are presented
in~\cref{lem:hb-invariant}.
Given two timestamps $T_1$ and $T_2$, we use the notation 
$T_1 \mx T_2$ to denote the timestamp $\lambda t, \max\set{T_1(t), T_2(t)}$; see for example
\cref{line:HB-read-LRFArr} and~\cref{line:HB-read-RMW} in~\cref{algo:hb-timestamps}.
\begin{description}
	\item[$\Hh_t$] For every thread $t$, the algorithm maintains a variable $\Hh_t$.
	Informally, $\Hh_t$ stores the timestamp $\HB_{\event_t}$,
	where $\event_t$ is the last event of event $t$ processed by the algorithm at a given time.
	\item[$\LRFH_t$] For every thread $t$, the algorithm maintains a variable $\LRFH_t$.
	The algorithm tracks the the $\hb$-timestamp of the last fence event
	$\event_t$ in $t$ for which $\event_t.\ord \sqsupseteq \MOrel$, and over-writes it with the timestamp
	of the latest event of thread $t$ if this latest event is a write or RMW event with strength higher or equal to $\MOrel$.
	This is used it to determine
	$\sw$ edges necessarily for computing the $\hb$ partial order.
	\item[$\SW_t$] For every thread $t$, the algorithm maintains a variable $\SW_t$, which stores a timestamp (i.e., vector indexed by threads).
	At a give point in the algorithm, the value $\SW_t[u]$ points to the latest event $\event_u$
	of thread $u$ for which $(\event_t, \event_u)$ is either a \emph{partial} $\sw$ edge, possibly preceded by an $\hb$-path.
	The algorithm tracks these timestamps to infer complete $\sw$ edges and thus the $\hb$ partial order.
	\item[$\LRFArr$] The algorithm maintains an event-indexed array $\LRFArr$ of timetamps.
	For a write, RMW or a fence event $\event$ (with $t = \event.\tid$), 
	we have $\LRFArr[\event] = \HB_f$, where $f$ is the latest fence operation
	with strength higher or equal to $\MOrel$.
	This is used to infer $\hb^?;\sw$ predecessors of acquire reads/RMWs/fences that appear later.
	\item[$\Uu$] This array, again indexed by events, stores timestamps.
	For an RMW event $\event$, $\Uu[\event]$ at a given point, stores the cumulative $\hb$-timestamps of the writes (if they are release writes) or their $\po$-predecessor release fences (otherwise) in the RMW chain of $\event$.
\end{description}


\newcommand{\lst}{\mathsf{last}}
\newcommand{\lsti}[1]{{(#1),\lst}}
\newcommand{\relfence}{\fnc,\MOrel}
\newcommand{\locIdx}{\mathsf{locIdx}}

We now formally state the invariants maintained by \cref{algo:hb-timestamps} in \cref{lem:hb-invariant}.
These invariants are established using induction.
Further, \cref{thm:HB-computation} follows as a corollary of \cref{lem:hb-invariant}.

For an event $\event$ of thread $t$, we use the notation
$\locIdx(\event) = |\setpred{f}{(f, \event) \in \po^?}|$ to denote the position of $\event$ within its own thread.
It follows that $\HB_{\event}(u) = \max\setpred{\locIdx(f)}{(f, \event) \in \hb^?}$.
We use the shorthand $\E_t$ to denote the set $\setpred{\event \in \E}{\event.tid = t}$.
In the same vein, the set $\E_t^{\sqsupseteq \MOrel}$ will denote the set
$\E_t \cap \E^{\sqsupseteq \MOrel}$.
For a sequence $\sigma$ of events, we use $\lst(\sigma, S)$ to denote the last
event in $\sigma$ which belongs to the set $S$. 
For example, $\lst(\sigma, \F^{\sqsupseteq \MOrel}_{t})$ to denote the last event $\event \in \sigma$
such that $\event.\tid = t$, $\event.\op = \fnc$ and $\event.\ord \in \set{\MOrel, \MOacqrel}$.

\begin{restatable}{lemma}{HB-invariant}\label{lem:hb-invariant}
Let $\E$, $\po$ and $\rf$ be inputs to  \cref{algo:hb-timestamps} 
such that $(\po \cup \rf)$ is acyclic.
Let $\pi = \event_1, \event_2 \ldots, \event_n$ 
be the sequence in which \cref{algo:hb-timestamps} processes the events of $\E$.
Let $i \geq 0$, let $\pi_i = \event_1, \ldots, \event_i$ be the prefix of $\pi$ of length $i$ (with $\pi_0 = \epsilon$).
% For a thread $t$, 
% let $e^\lsti{i}_t$ denote the last event $e$ in $\pi_i$ for which $e.\tid = t$.
% and let $e^{\lsti{i}}_{t, \relfence}$ be the
% last event $e$ in $\pi_i$ for which $e.\tid = t$, $e.\op = \fnc$ and $e.\ord = \MOrel$.
Further, let $\Hh_t^{(i)}$, $\LRFH_t^{(i)}$, $\SW_t^{(i)}$, $\Uu^{(i)}$,
$\HB^{(i)}$ and $\LRFArr^{(i)}$ be the values of 
respectively $\Hh_t$, $\LRFH_t$, $\SW_t$, $\Uu$,
$\HB$ and $\LRFArr$ 
after having processed the prefix $\pi_i$. 
We have the following.
\begin{compactenum} 
	\item\label{item:HB-Hh} $\Hh_t^{(i)} = \HB_\event$, where $\event = \lst(\pi_i, \E_t)$. 
	If no such $\event$ exists in $\pi_i$, then $\Hh_t^{(i)} = \lambda u, 0$.

	\item\label{item:HB-HB} For an $\event \in \pi_i$, $\HB^{(i)}[\event] = \HB_{\event}$. 
	% \item\itmlabel{HB-LRFH} $\LRFH_t^{(i)} = \HB_e$, where $e = \lst(\pi_i, \F^{\sqsupseteq \MOrel}_{t})$.

	\item\label{item:HB-LRFH} 
	$\LRFH_t^{(i)} = \HB_\event$, where $\event = \lst(\pi_i, \F^{\sqsupseteq \MOrel}_t)$. 
	If no such $\event$ exists in $\pi_i$, then $\LRFH_t^{(i)} = \lambda u, 0$.
	% \[
	% \LRFH_t^{(i)} = 
	% \begin{cases}
	% 	\HB_e & \text{ if } e = \lst(\pi_i, \E^t) \text{ exists}, e.\op \in \set{\wt, \ud} \text{ and } e.\ord \sqsupseteq \MOrel \\
	% 	\HB_e & \text{ otherwise, if } e =  \lst(\pi_i, \F_{\sqsupseteq \MOrel}^{t}) \text{ exists} \\
	% 	\lambda u, 0 & \text{ otherwise}
	% \end{cases}
	% \]

	\item\label{item:HB-LRFArr} For each $\event \in \pi_i$,
	 such that $\event.\op \in \set{\wt, \ud}$, 
	\[
	\LRFArr^{(i)}[\event] = 
	\begin{cases}
		\HB_{f} & \text{ such that } f = \lst(\pi_i, \F^{\sqsupseteq \MOrel}_t) \text{ where } t = \event.\tid \\
		\lambda u, 0 & \text{ otherwise if no such $f$ exists}
	\end{cases}
	\]
	% \[
	% \LRFArr^{(i)}[e] = 
	% \begin{cases}
	% 	\HB_e & \text{ if } e.\ord \sqsupseteq \MOrel \\
	% 	\HB_f & 
	% 	\text{ otherwise if } 
	% 	\begin{array}{c}
	% 	f \text{ is the last event with } \\
	% 	(f, e) \in \po, f.\op = \fnc, f.\ord \sqsupseteq \MOrel
	% 	\end{array} \\
	% 	\lambda u, 0 & \text{ otherwise if no such $f$ exists}
	% \end{cases}
	% \]
	If $\event.\op \not\in \set{\wt, \ud}$ then $\LRFArr^{(i)}[\event]$ is undefiend.
	\item\label{item:HB-SW} $\SW_t^{(i)}[u] = \locIdx(\event)$, where $\event$ is the last event in $\pi_i$
	such that $\event.\tid = u$ and $(\event, \lst(\pi_i, \E_t)) \in \hb^?;[\E^{\sqsupseteq \MOrel}];([\F];\po)^?;\rf^+;\po^?$.
	If no such $\event$ exists, then $\SW_t^{(i)}[u] = 0$. \\
	Observe that since $\pi_i$ is consistent with $\hb \subseteq (\po \cup \rf)^+$,
	if $\event$ exists in $\pi$, then it exists in $\pi_i$ too.
	\item\label{item:HB-RMW} For an event $\event \in \pi_i$ such that $\event.\op = \ud$,
	$\Uu^{(i)}[\event][t] = \locIdx(f)$, where $f$ is the last event in $\pi$
	such that $f.\tid = t$ and $(f, \event) \in \hb^?;[\E^{\sqsupseteq \MOrel}];([\F];\po)^?;\rf^+$ --- notice that
	we require that the path from $f$ to $\event$ ends in an $\rf$ edge and not a $\po$ edge.
	If no such $f$ exists, then $\Uu^{(i)}[\event][t] = 0$. \\
	As before, since $\pi_i$ is consistent with $\hb \subseteq (\po \cup \rf)^+$,
	if $f$ exists in $\pi$, then it exists in $\pi_i$ too. \\
	If $\event.\op \neq \ud$ then $\Uu^{(i)}[\event]$ is undefiend.
\end{compactenum}
\end{restatable}

\begin{proof}
We prove the above invariants by induction on the length $i$ of the prefix processed by the algorithm.
In the base case $(i = 0)$, the invariants \cref{item:HB-HB}, \cref{item:HB-LRFArr} and \cref{item:HB-RMW} vacuously hold as there in no $\event \in \pi_i$. 
The other three invariants also hold because the corresponding clocks $\Hh_t$, $\LRFH_t$ and $\SW_t$ are initialized with $\lambda u. 0$.

Let us consider the inductive case. 
Assume that all the invariants
\cref{item:HB-Hh}, \cref{item:HB-HB}, \cref{item:HB-LRFH}, \cref{item:HB-LRFArr}, 
\cref{item:HB-SW} and \cref{item:HB-RMW} hold for the prefix $\pi_i = \event_1, \event_2, \ldots, \event_i$, 
and we argue that hold for the prefix $\pi_{i+1} = \pi_i e_{i+1}$.
Let $t = \event_{i+1}.\tid$.
First we argue that the timestamps corresponding to all 
previous events remain unchanged in the new prefix $\pi_{i+1}$.
The $\HB$-timestamp of an event $\event$ only depend upon events that are $(\po\cup\rf)^+$-before $\event$
and thus must precede $\event$ in $\pi_{i+1}$.
Likewise, $\LRFArr[\event] = f$ implies that $f$ must be $\po^?$-before $\event$ and thus must appear prior to $\event$ in $\pi_{i+1}$.
Similarly, $\Uu^{(i)}[\event][t] = \locIdx(f)$ implies that $f$ is $(\po\cup\rf)^+$-before $\event$ and thus must appear prior to $\event$ in $\pi_{i+1}$.
We can similarly argue that the value of all clocks associated with a thread $u \neq t$ must remain unchanged
because they record information about some event of the form $\event = \lst(\pi_i, \E^u)$ or $\event = \lst(\pi_i, \F^{\sqsupseteq \MOrel}_{u})$, and events that are  $(\po\cup\rf)^+$-before $\event$. 
Since $\event$ appears in $\pi_i$ (because $u \neq \event_{i+1}.\tid$), it must be that all these clocks remain unchanged.
Thus, we only need to argue about the entries corresponding to $\event_{i+1}$
and how the clocks with subscript $t$ change.

We will do a case-by-case analysis based on $\event_{i+1}.\op$.
Let us establish some notations and properties first.

Given some $j\in\{0,i-1\}$, let us define the set
\[
\E_{u, \SW_t, j} = \setpred{\event \in \pi_j}{\event.\tid = u, 
(\event, \lst(\pi_j, \E_t)) \in \hb^?;[\E^{\sqsupseteq \MOrel}];([\F];\po)^?;\rf^+;\po^?}\ .
\]
Observe that since events of a given thread (and thus the thread $t$ in particular) are $\po$-ordered,
we have $\E_{u, \SW_t, j} \subseteq \E_{u, \SW_t, k}$ if $j \leq k$.
Thus, $\E_{u, \SW_t, i} \subseteq \E_{u, \SW_t, i+1}$.
Let us now establish the following equation
\begin{equation}
\label{eq:SW_t_induction}
\E_{u, \SW_t, i+1} = \E_{u, \SW_t, i} \cup S_{\mathsf{rf}}(\event_{i+1}) \cup S_{\rf^+}(\event_{i+1})
\end{equation}
where
\[
\begin{array}{rcl}
S_{\mathsf{rf}}(\event) &=& \setpred{f}{\event.\op \in \set{\rd, \ud}, f.\tid = u, (f, \rf(\event)) \in  \hb^?;[\E^{\sqsupseteq \MOrel}];([\F];\po)^?} \\
S_{\mathsf{rf}^+}(\event) &=& \setpred{f}{\event.\op = \ud, f.\tid = u, \rf(\event).\op = \ud, (f, \rf(\event)) \in  \hb^?;[\E^{\sqsupseteq \MOrel}];([\F];\po)^?;\rf^+}
\end{array}
\]
First observe that $\E_{u, \SW_t, i} \subseteq \E_{u, \SW_t, i+1}$, 
$S_{\mathsf{rf}}(\event_{i+1}) \subseteq \E_{u, \SW_t, i+1}$ and 
$S_{\mathsf{rf}^+}(\event_{i+1}) \subseteq \E_{u, \SW_t, i+1}$ and thus we need to only establish that
$\E_{u, \SW_t, i+1} \subseteq \E_{u, \SW_t, i} \cup S_{\mathsf{rf}}(\event_{i+1}) \cup S_{\mathsf{rf}^+}(\event_{i+1})$.
This follows using a simple case by case analysis on how the path 
$(\event, \event_{i+1})$ ends for a given $\event \in  \E_{u, \SW_t, i+1}$.
If it ends in a $\po$ edge, then $\event \in \E_{u, \SW_t, i}$.
If it ends in a single $\rf$ edge, then $\event \in S_{\mathsf{rf}}(\event_{i+1})$, and finally if it ends in a sequence of $\rf$ edges,
then $\event \in S_{\mathsf{rf}^+}(\event_{i+1})$.

\newcommand{\HBBef}{\textsf{HBBef}}
Now, for an event $\event$, let $\HBBef(\event) = \setpred{f}{(f, \event) \in \hb^?}$.
If $\event$ does not exist, then we let $\HBBef(\event) = \emptyset$.
Let us establish the following equation:
\begin{equation}
\label{eq:HB_induction}
\HBBef(\event_{i+1}) = 
\set{\event_{i+1}} \cup \HBBef(\event^{\po}_{i+1}) \cup S_{\MOacq, \rd}(\event_{i+1}) \cup  S_{\MOacq, \fnc}(\event_{i+1})
\end{equation}
where
$\event_{i+1}^\po$ is the unique event with $(\event^{\po}_{i+1}, \event_{i+1}) \in \po_\imm$,
\[
\begin{array}{rcl}
S_{\MOacq, \rd}(e) &=& \setpred{f}{\event.\ord \sqsupseteq \MOacq, f \in S_{\mathsf{rf}}(e) \cup S_{\mathsf{rf}^+}(e)} \\
S_{\MOacq, \fnc}(e) &=& \setpred{f}{\event.\ord \sqsupseteq \MOacq, \event.\op = \fnc, \exists g, (g, e) \in \po, f \in S_{\mathsf{rf}}(g) \cup S_{\mathsf{rf}^+}(g)}
\end{array}
\]
The above equation follows because if $(f, \event_{i+1}) \in \hb^?$, then either $f = \event_{i+1}$, or
there is an event $g$ such that $(f, g) \in \hb^?$ and either (a) $(g, \event_{i+1}) \in \po$, or (b) $(g, \event_{i+1}) \in \sw$.
In the former case, we can take $g = \event^\po_{i+1}$.
In the latter case, we have $(g, \event_{i+1}) \in [\E^{\sqsupseteq \MOrel}];([\F];\po)^?;\rf^+;(\po;[\F])^?;[\E^{\sqsupseteq \MOacq]}]$ and thus $\event_{i+1}.\ord \sqsupseteq \MOacq$.
If $\event_{i+1}.\op \in \set{\rd, \ud}$, then it is easy to see that $f \in S_{\MOacq, \rd}(\event_{i+1})$.
If on the other hand $\event_{i+1}.\op = \fnc$, then it is easy to see that $f \in S_{\MOacq, \fnc}(\event_{i+1})$.


\begin{compactdesc}
	\item[Case $\event_{i+1}.\op = \rd$.] 
	First, observe that $\lst(\pi_i, \F^{\sqsupseteq \MOrel}_{t}) = \lst(\pi_{i+1}, \F^{\sqsupseteq \MOrel}_{t})$ and thus $\LRFH_t^{(i+1)} = \LRFH_t^{(i)}$.

	Next we consider $\SW^{(i+1)}_t[u]$ for some thread $u$.
	First, if $\SW^{(i+1)}_t[u] = 0$, then observe that
	$\E_{u, \SW_t, i+1} = \emptyset$.
	From \cref{eq:SW_t_induction}, it follows that
	$\E_{u, \SW_t, i} = S_{\mathsf{rf}}(\event_{i+1}) = \emptyset$, and further, if $w = \rf(\event_{i+1})$ is an RMW, then $S_{\mathsf{rf}^+}(\event_{i+1}) = \emptyset$.
	In this case, the updates in \cref{line:HB-read-LRFArr-SW} and \cref{line:hb-read-end}
	correctly reflect the value of $\SW^{(i+1)}_t[u]$.
	Next, we consider the case when $\SW^{(i+1)}_t[u] = m > 0$

	Let $\event$ be the event such that $\event.\tid = u$ and $\locIdx(e) = m = \SW^{(i+1)}_t[u]$.
	First, we observe that $\event \in \E_{u, \SW_t, i+1}$ and thus
	we have one of (a)~$\event \in \E_{u, \SW_t, i}$, or (b) $\event \in S_{\mathsf{rf}}(\event_{i+1})$ or (c) $\event \in S_{\mathsf{rf}^+}(\event_{i+1})$.
	By induction we will have respectively (a) $\SW^{(i)}_t[u] \geq m$,
	(b)~$\LRFArr[w][u] \geq m$, where $w = \rf(\event_{i+1})$, and 
	(c)~$w.\op = \ud$ with $\Uu[w][u] \geq m$.
	In each of these cases, if the inequality is strict (i.e., $> m$), then
	we know that there is another event $\event'$ such that $(\event, \event') \in \po$ and
	one of $\event' \in \E_{u, \SW_t, i}$, or $\event' \in S_{\mathsf{rf}}(\event_{i+1})$ or $\event' \in S_{\mathsf{rf}^+}(\event_{i+1})$ holds,
	and thus $\event' \in \in \E_{u, \SW_t, i+1}$ implying that 
	$\SW^{(i+1)}_t[u] > m$ which is a contradiction.
	Thus, we have strict equality in one of (a) $\SW^{(i)}_t[u] \geq m$,
	(b) $\LRFArr[w][u] \geq m$, 
	(c) $\Uu[w][u] \geq m$.
	In this case, the updates in \cref{line:HB-read-LRFArr-SW} and \cref{line:hb-read-end}
	correctly reflect the value of $\SW^{(i+1)}_t[u]$.

	Now, we argue about $\Hh_t$.
	Here, $S_{\MOacq, \fnc}(\event_{i+1}) = \emptyset$ since $\event_{i+1}.\op \neq \fnc$.
	Thus, we have $\HBBef(\event_{i+1}) = \set{\event_{i+1}} \cup \HBBef(\event^{\po}_{i+1}) \cup S_{\MOacq, \rd}(\event_{i+1})$.
	As with $\SW_t$, we can argue that $\Hh_t^{(i+1)}$ is correctly updated.	


	Next, $\HB[{\event_{i+1}}] = \HB_{\event_{i+1}}$ follows because $\event_{i+1} = \lst(\pi_{i+1}, \E_t)$.

	Finally, since $\event_{i+1}.\op \neq \ud$, $\Uu[\event_{i+1}]$ is undefined as also ensured by the algorithm.

	\item[Case $\event_{i+1}.\op = \wt$.] 
	In this case, $\lst(\pi_i, \F^{\sqsupseteq \MOrel}_{t}) = \lst(\pi_{i+1}, \F^{\sqsupseteq \MOrel}_{t})$ and thus $\LRFH_t^{(i+1)} = \LRFH_t^{(i)}$.
	Finally, $\LRFArr[\event_{i+1}] = \LRFH_t^{(i+1)}$ as expected.

	Now, we consider $\SW^{(i+1)}_t[u]$ for some thread $u$.
	Recall $\E_{u, \SW_t, i+1} = \E_{u, \SW_t, i} \cup  S_{\mathsf{rf}}(\event_{i+1}) \cup S_{\rf^+}(\event_{i+1})$.
	Since $\event_{i+1}.\op = \wt$, we have 
	$\E_{u, \SW_t, i+1} = \E_{u, \SW_t, i}$.
	It follows that $\SW^{(i+1)}_t[u] = \SW^{(i)}_t[u]$ and this is what the algorithm ensures.

	Finally, we consider $\Hh_t^{(i+1)}$.
	Recall that $\HBBef(\event_{i+1}) = \set{\event_{i+1}} \cup \HBBef(\event^{\po}_{i+1}) \cup S_{\MOacq, \rd}(\event_{i+1}) \cup  S_{\MOacq, \fnc}(\event_{i+1})$.
	Since $\event.\op \not\in \set{\rd,\ud,\fnc}$, we have 
	$\HBBef(\event_{i+1}) = \set{\event_{i+1}} \cup \HBBef(\event^{\po}_{i+1})$ and the algorithm ensures this.

	Finally, since $\event_{i+1}.\op \neq \ud$, $\Uu[\event_{i+1}]$ is undefined as also ensured by the algorithm.

	\item[Case $\event_{i+1}.\op = \ud$.] 
	This case follows from the above two cases, except for $\Uu[\event_{i+1}]$. We will argue about $\Uu[\event_{i+1}]$ next.
	Consider an event $f$ such that $(f, \event_{i+1}) \in \hb^?;[\E^{\sqsupseteq \MOrel}];([\F];\po)^?;\rf^+$.
	We have two cases.
	
	First, there is only a single trailing $\rf$ edge, i.e.,
	$(f, \event_{i+1}) \in \hb^?;[\E^{\sqsupseteq \MOrel}];([\F];\po)^?;\rf$.
	In this case, $f \in S_{\mathsf{rf}}(\event_{i+1})$.
	Otherwise, we have $(f, \event_{i+1}) \in \hb^?;[\E^{\sqsupseteq \MOrel}];([\F];\po)^?;\rf^+;\rf$.
	In this case, $\rf(\event_{i+1}).\op = \ud$ and further $f \in S_{\mathsf{rf}}(\rf(\event_{i+1}))$.
	The correctness then follows.


	\item[Case $\event_{i+1}.\op = \fnc$]
	Recall that $\HBBef(\event_{i+1}) = \set{\event_{i+1}} \cup \HBBef(\event^{\po}_{i+1}) \cup S_{\MOacq, \rd}(\event_{i+1}) \cup  S_{\MOacq, \fnc}(\event_{i+1})$.
	Since $\event.\op \not\in \set{\rd,\ud}$, we have 
	$\HBBef(\event_{i+1}) = \set{\event_{i+1}} \cup \HBBef(\event^{\po}_{i+1}) \cup  S_{\MOacq, \fnc}(\event_{i+1})$.
	Consider an event $\event$ such that $\event \in  S_{\MOacq, \fnc}(\event_{i+1})$.
	This means that there is a $g$ such that $(g, \event_{i+1}) \in \po$ and 
	$(\event, g) \in S_{\mathsf{rf}}(g) \cup S_{\rf^+}(g)$.
	This in turn means that 
	$(\event, \rf(g)) \in  \hb^?;[\E^{\sqsupseteq \MOrel}];([\F];\po)^?;\rf^*$.
	Thus, $(\event, \event_{i+1}) \in  \hb^?;[\E^{\sqsupseteq \MOrel}];([\F];\po)^?;\rf^+;\po$.
	Thus, $\SW_t^{i}[\event.\tid] \geq \locIdx(\event)$ by induction.

	Next, $\LRFArr[\event_{i+1}]$ is undefined since $\event_{i+1} \not\in \set{\wt, \ud}$.
	Finally, $\LRFH_t^{i+1} = \HB_{\event_{i+1}}$ since $\event_{i+1}.\op = \fnc$ and $\event_{i+1} = \lst(\pi_{i+1}, \E_t)$.
\end{compactdesc}
\end{proof}



%\bparagraph{Computing $\glw$ and $\glr$}
%\cref{algo:last-write-before} presents the pseudocode for initializing 
%and accessing the data structures $\view{\WtLst}{t,x}{u}$ and $\view{\RdLst}{t,x}{u}$
%(one for every $t, x, u$) used for
%computing the values of the $\glw(t, x, c)$ and $\glr(t, x, c)$ functions.
%\input{algorithms/algo-lastWrite}
%
%
%
%\bparagraph{Top of, and relative position in  $\rf$-chain}
%Finally, we refer to \cref{algo:tc-pc} that computes the maps $\TC$ and $\PC$.
%\input{algorithms/algo-tc-pc}




==> app_scalability_tex.tex <==
\subsection{Synthetic Benchmarks}
\label{sec:experiment-synthetic}
In this section we discuss various hand crafted benchmarks to showcase the different features of \cref{algo:ra-rf-on-the-fly} and \celeventester algorithm in a controlled experimental setting. 
The benchmarks are created to exhibit certain behaviors which exploit contrasting aspects of the algorithms.
It is aimed that these benchmarks provide a better understanding of the algorithm by demonstrating when and why \cref{algo:ra-rf-on-the-fly} ensues a better performance.
The standard benchmarks found in the literature typically contain complex and convoluted behaviors which prevent from conducting such detailed analysis.    
The examples provided in \cref{sec:synthetic-bench-rmw-rw} and \cref{sec:synthetic-bench-rmw-wr} harness the features discussed in \cref{sec:efficient-rmw-handling}, and the examples provided in \cref{sec:synthetic-bench-r-partial-satur} and \cref{sec:synthetic-bench-no-w-satur} harness the features discussed in  \cref{sec:no-prop-across-threads} and \cref{sec:no-saturation-write}, respectively. The example discussed in \cref{sec:synthetic-bench-hb-aware} discusses one of the disadvantages of \cref{algo:ra-rf-on-the-fly}.



\subsubsection{Fixed RMW Chain Read-Write}
\label{sec:synthetic-bench-rmw-rw}
Consider the execution depicted in \cref{subfig:fixed-rmw-chain-rw}.
In this execution the program first executes the write event $\event_1$ in thread $t$ and then spawns the threads $t_i$ for $i \in [1, k]$.
The threads $t_1\ldots t_k$ perform a read event followed by a write event in these threads.
The read events are always reading from the first write event in thread $t$.
This results in an $\mo$ edge to be formed from $\event_1$ into the write events in the threads $t_1\ldots t_k$.
Then, the program executes the RMW events in thread $t$  where the RMW events are always reading from their $\po$ predecessor. 
This results in an RMW chain of length $n$ where $n$ is the number of events executed by thread $t$. 
Observe that during the initialization of each RMW event it is normally required to infer the $\mo$ edge from the current RMW event into the write events in the other threads $t_1\ldots t_k$ due to the existing $\mo$ edge from $\event_1$ into the write events in the other threads (see \cref{subfig:rmw-infer-2}).
This would result in inferring $(n-1)\times k$ many $\mo$ edges.
As discussed in \cref{sec:efficient-rmw-handling}, \cref{algo:ra-rf-on-the-fly} does not explicitly infer these edges. 
This benchmark is constructed with the aim of demonstrating that \cref{algo:ra-rf-on-the-fly} is able to efficiently handle such scenarios that involve adding outgoing $\mo$ edges from RMW events. 


\subsubsection{Fixed RMW Chain Write-Read}
\label{sec:synthetic-bench-rmw-wr}
Consider the execution depicted in \cref{subfig:fixed-rmw-chain-wr}.
In this execution the program first executes all the events in thread $t$ and obtains an RMW chain of length $n$ where $n$ is the number of events executed by thread $t$.
Then, the program spawns the threads $t_i$ for $i \in [1, k]$ and these threads perform a write event followed by a read event.
The read events are always reading from the last RMW event in thread $t$.
This results in an $\mo$ edge to be formed from the write events in threads $t_1 \ldots t_k$ into the last RMW event in thread $t$.
Observe that adding such an edge requires inferring an $\mo$ edge to the head of the RMW chain (see \cref{subfig:rmw-infer-1}).
Therefore, the new incoming $\mo$ edges from the write events in the threads $t_1 \ldots t_k$ should normally be propagated into all the events in the RMW chain.
This benchmark is constructed with the aim of demonstrating that \cref{algo:ra-rf-on-the-fly} efficiently represents the incoming $\mo$ edges to all the events in an RMW chain as a single $\HBMO$ clock.
This enables \cref{algo:ra-rf-on-the-fly} to efficiently handle such scenarios that involve incoming $\mo$ edges to the RMW events.


\subsubsection{Partial Saturation for New Read Events}
\label{sec:synthetic-bench-r-partial-satur}
Consider the execution depicted in \cref{subfig:partial-satur-read}. 
This execution contains two locations.
The program first executes the events $\event_1$ and $\event_2$ in thread $t'$ and then executes all the events in thread $t$.
Executing the read event $\event_3$ in thread $t$ results in $\mo$ edges to be formed from the write event $\event_1$ in thread $t'$ into all the write events in thread $t$.
Then, the threads $t_i$ are spawned for $i \in [1, k]$.
These threads first execute a write event followed by a read event.  
The read events in the threads $t_1\ldots t_k$ are always reading from the write event $\event_1$ in thread $t'$.
This results in adding an $\mo$ edge from the write events in the threads $t_1 \ldots t_k$ into the event $\event_1$. 
Observe that the new incoming $\mo$ edge should normally be propagated into all the write events in the thread $t$ due to the existing $\mo$ edge from $\event_1$ into all the write events in thread $t$.
This benchmark is constructed with the aim of demonstrating that \cref{algo:ra-rf-on-the-fly} does not propagate $\mo$ edges across different threads. 
Therefore, this leads \cref{algo:ra-rf-on-the-fly} to efficiently handle such scenarios.   

\subsubsection{No Write Saturation}
\label{sec:synthetic-bench-no-w-satur}
Consider the execution depicted in \cref{subfig:no-write-satur}. 
This execution contains two locations.
The program first executes all the events in thread $t$.
This results in an $\mo$ chain of length $n$ to be formed where $n$ is the number of write events executed by thread $t$ on location $x$.
Then, the read event $\event_5$ in thread $t'$ is executed which results in an $\hb$ edge to be formed between thread $t$ and $t'$.
Afterwards, all the write events are executed in thread $t'$.
Observe that normally processing each of these write events performed in thread $t'$ requires fetching the last $\hb$ write in thread $t$.
This benchmark is constructed with the aim of demonstrating that \cref{algo:ra-rf-on-the-fly} does not perform saturation when it observes new write events. Therefore, this leads to an efficient procedure for handling new write events.   


\subsubsection{HB Aware}
\label{sec:synthetic-bench-hb-aware}
Consider the execution depicted in \cref{subfig:hb-aware}. 
The execution starts by spawning the threads $t_i$ for $i \in [1, k]$.
Then, $k$-many read events are executed in thread $t$ and these read events read from the write events in threads $t_i \ldots t_k$ such that these write events are read from exactly once.  
Afterwards, an RMW chain of length $n$ is formed in thread $t$.
For processing each RMW event, \cref{algo:ra-rf-on-the-fly} iterates over all threads and fetches the last write event performed by each thread which is $\hb$-ordered before the current RMW event.
This amounts to fetching $k$ many write events and then updating the respective $\HBMO$ clocks (\cref{line:ra-otf-check-end}).
Observe that if the $\HBMO$ clocks of write events were transitively closed then one does not need to consider the write events of which the current RMW event is $\hb$ aware.
However, \cref{algo:ra-rf-on-the-fly} does not keep this relation transitively closed, hence, it cannot straightforwardly ignore such events. 
This benchmark is constructed with the aim of evaluating this side effect of \cref{algo:ra-rf-on-the-fly}.   


==> app_sra_rf_np_hard.tex <==
\subsection{Proof of {\cref{thm:sra_rf_lower}}}\label{subsec:app_SRA-RMW-RF-Consistency-NP-Hard}


%\SCRMWRFConsistencyNPHardwriteobservedonce*
%\begin{proof}
%Given an instance $\expartial=(\E, \po, \rf)$ of the consistency problem for $\scmm$, where 
%(i)~$\E$ contains only read and write events, and
%(ii)~$\rf$ is bijective,
%we construct an instance $\expartial'=(\E', \po', \rf')$ of the consistency problem for $\scmm$ as follows.
%For every read event $\rd \in \E^{\R}$, we have an RMW event $\ud_\rd\in \E^{\U}$
%such that $\ud_\rd.\id = \rd.\id$, $\ud_\rd,\tid = \rd.\tid$, $\ud_\rd.\lloc = \rd.\lloc$,
%and replace all occurrences of $\rd$ by $\ud$ in $\ex'$.
%That is, $\ex'.\E = \ex.\E \setminus \ex.\R \cup \setpred{\ud_\rd}{\rd \in \ex.\R}$.
%Similarly, $\ex'.\po = \ex.\po \cap (\ex'.\E \times \ex'.\E) \cup \setpred{(e, \ud_\rd)}{(e, \rd) \in \ex.\po, \rd \in \ex.\R} \cup \setpred{(\ud_\rd, e)}{(\rd, e) \in \ex.\po, \rd \in \ex.\R}$.
%Further,
%$\ex'.\rf = \setpred{(e, \ud_\rd)}{(e, \rd) \in \ex.\rf}$.
%That is, the read component of each newly introduced update event, 
%observes the same write event as observed by the original read event,
%while the write components of the update events are not observed by any event.
%Finally, note that since $\ex$ is such that every write event of $\ex$
%is observed by at most one read event, $\ex'$ also satisfies the same property.
%Now, it is easy to see that $\ex$ can be extended to an SC consistent execution
%iff $\ex'$ can be.
%\end{proof}

Given the above corollary, we can now prove \cref{thm:sra_rf_lower}.

\thmsrarflower*
\begin{proof}
Let $\ex$ be an instance of the RF consistency problem for SC with RMWs,
as in the statement
of \cref{cor:SC-RMW-RF-Consistency-NP-Hard-write-observed-once} 
(i.e., $\ex$ has no read events and every write event in $\ex$ is observed by at most one RMW event).
We construct $\ex' = \ex$ as the instance of RF consistency for SRA.
Observe that if $\ex$ is a positive instance, i.e., there is an $\mo$
for which $\ex$ is SC consistent, then the same $\mo$ also witnesses the SRA consistency 
of $\ex' = \ex$.
Next, assume that $\ex' = \ex$ is RF consistent for the SRA fragment
and let $\mo$ be the witness coherence order on all the write and update events.
Since, $\ex'$ is such that every write is observed at most once and 
all the $\rf$ edges are directed to RMW events,
we have $\fr \subseteq \mo$.
Now, SRA consistency of $\ex'$ ensures that $(\hb \cup \mo)$ is acyclic
and thus we have $(\po \cup \rf \cup \mo \cup \fr)$ is acyclic.
This means that $\ex = \ex'$ is also SC consistent with the same choice of $\mo$.
\end{proof}

==> consistency_axioms.tex <==
\subsection{Consistency Axioms}\label{subsec:consistency_axioms}

Consistency axioms characterize different aspects or constraints of 
the underlying memory model.
We broadly classify these constraints as 
coherence, atomicity, global ordering, and causality cycles.  
Different interpretations of these constraints give rise to different consistency models.

\bparagraph{Coherence}
In an execution, coherence enforces \emph{SC-per-location}: the memory accesses per memory locations are totally ordered. 
We may also further categorize coherence as 
write-coherence and read-coherence. 
\emph{Write-coherence} enforces that $\mo$ agrees with $\hb$. 
Another variation is \emph{strong-write-coherence}, which requires that this condition holds transitively.
Read coherence enforces that a read $\rd(x)$ cannot read from a write $\wt(x)$ if 
there is an \emph{intermediate} write $\wt(x)'$ that happens-before $\rd(x)$, 
i.e. $\hb(\wt(x)',\rd(x))$ holds.
Depending on the precise notion of ``intermediate'', we obtain two variants~\cite{Lahav:2022}:~\emph{read-coherence}, where intermediate is wrt $\mo$ (i.e., we have $\mo(\wt'(x),\wt(x))$), and
\emph{weak-read-coherence}, where intermediate is wrt $\hb$ (i.e., we have $\hb(\wt'(x),\wt(x))$).
We list the formal definitions of the various coherence axioms below. 
\begin{compactitem}
%\item $(\poloc \cup \rf \cup \mo \cup \fr)$ is acyclic. \hfill (SC-per-location)
\item $(\mo;\rf^?;\hb^?)$ is irreflexive.  \hfill (write-coherence) 
\item $(\hb \cup \mo)$ is acyclic. \hfill (strong-write-coherence) 
\item $(\fr;\rf^?;\hb)$ is irreflexive. \hfill (read-coherence)
\item $(\hbloc;[\W \cup \U];\hb;\rf^{-1})$ is irreflexive. \hfill (weak-read-coherence)
\end{compactitem}
%Going forward we define memory models that vary based on their respective coherence axioms. 

\bparagraph{Atomicity}
The property ensures that the (successful) RMW accesses in an execution indeed update the memory locations atomically. 
Following~\cite{Lahav:2022}, we consider two variants. 
\emph{Atomicity} ensures that no intermediate write event 
on the same location takes place between an RMW and its writer.
%For example, suppose $u$ is an update event and $w$ is a write on the same location that violates atomicity. 
%In that case $\fr(u,w)$ as well as $\mo(w,u)$ hold. Axiom (atomicity) restricts it. 
On the other hand, \emph{weak-atomicity} simply prohibits two RMW events to have the same writer.
\begin{compactitem}
\item $\fr;\mo$ is irreflexive. \hfill (atomicity)
\item $\forall \ud_1, \ud_2\in \U, \rf(\ud_1)\neq \rf(\ud_2)$. \hfill (weak-atomicity)
%\item $\forall (w_1, \event_1), (w_2, \event_2) \in \rf;[\U].~ w_1 = w_2 \implies \event_1 = \event_2$ \hfill (weak-atomicity)
\end{compactitem}

%\bparagraph{Global Ordering}
%Coherence and atomicity enforce ordering constraints on same-memory location accesses. 
%In the concurrency models we consider here, additional orderings are imposed
%between fence operations or memory accesses on different memory locations, primarily due to $\hb$.
%The following axiom, integral to many memory models, enforces that an event cannot happen-before itself.
% Using $\hb$ relation we ensure that in an execution an event cannot happen-before itself by using the following axiom.
%\begin{compactitem}
%\item $\hb$ is irreflexive. \hfill (irrHB) 
%\end{compactitem} 
% In addition, certain C/C++ concurrency models use relation 
% $\SC$ to obtain a global ordering as $\SC$ is a total order on all $\MOsc$ accesses. \ucomment{remove?}

\bparagraph{Causality Cycles} 
A causality cycle arises in presence of primitives that have weaker behaviors than release-acquire accesses. 
Such a cycle consists of $\po$ and $\rf$ orderings and may result in 
`out-of-thin-air' behavior in certain programs. 
To avoid such `out-of-thin-air' behavior, many consistency models 
explicitly disallow such cycles.
\begin{compactitem}
\item $(\po \cup \rf)$ is acyclic. \hfill (PO-RF) 
\end{compactitem}
In the absence of $\MOrlx$ accesses, the PO-RF axiom coincides with the requirement for $\hb$ acyclicity~\cite{Lahav:2022}.


==> consistency_models.tex <==
\subsection{Axiomatic Consistency Models} 

We are now in position to present the memory models we consider in this work.
For the sake of completeness, we also state Sequential Consistency as a standard reference model.

\bparagraph{Sequential Consistency}
%While we do not consider Sequential Consistency (SC) memory model in this work, we define it for the sake of completeness.
Sequential consistency ($\scmm$) enforces a global order on all memory accesses. 
This is a stronger constraint than coherence which orders same-location memory accesses. 
In addition, $\scmm$ also guarantees atomicity. 
%The precise axiomatic specification of SC is as follows. 
\begin{compactitem}
\item $\ (\po \cup \rf \cup \mo \cup \fr)$ is acyclic. \hfill ($\scmm$)
\end{compactitem}

\bparagraph{Release-Acquire and variants}
The release-acquire memory model is weaker than SC, 
and is arguably the most well-understood fragment of C11. 
Broadly, under the release-acquire semantics (including other related variants),
each read-from ordering establishes a synchronization. 
In this case, the relation $\hb \triangleq(\po \cup \rf)^+$ has a 
simpler description in presence of release-acquires accesses only. 
Following~\cite{Lahav:2022}, we consider three variants of 
release-acquire models: $\ramm$, strong RA ($\sramm$), and weak RA ($\wramm$). 

First, we consider the basic $\ramm$ memory model.
% RA enforces coherence by (write-coherence) and (read-coherence), atomicity property by (atomicity) axiom, and global ordering by (irrHB).
\begin{compactitem}
\item (write-coherence) $\land$ (read-coherence) $\land$ (atomicity) \hfill ($\ramm$)
\end{compactitem}
Next, we consider $\sramm$, which enforces a stronger coherence guarantee
on write accesses compared to RA and ensures strong-write-coherence. 
Formally,
\begin{compactitem}
\item (strong-write-coherence) $\land$ (read-coherence) $\land$ (atomicity) \hfill ($\sramm$)
\end{compactitem}
Finally, we consider WRA, which does not place any restrictions on the $\mo$ ordering between same-location writes. 
Instead, the only orderings considered between same-location writes are through the $[\W];\hbloc;[\W]$ relation. 
As a result, WRA provides weaker constraints for coherence and atomicity by (weak-read-coherence) and (weak-atomicity) respectively:
\begin{compactitem}
\item (weak-read-coherence) $\land$ (weak-atomicity) $\land$ (PO-RF) \hfill ($\wramm$)
\end{compactitem}

\bparagraph{RC20}
The $\rcmm$ model is defined for the non-$\SC$ fragment in C/C++ concurrency that handles the semantics of relaxed accesses along with release-acquire primitives~\cite{Margalit:2021}.
It can nevertheless simulate $\scmm$ fences using release, acquire, and RMW primitives.
%RC20 provides coherence and atomicity guarantees by (write-coherence), (read-coherence), and (atomicity) axioms. 
%In addition, RC20 enforce (PO-RF) to avoid out-of-thin-air 
%behavior. 
\begin{compactitem}
\item (write-coherence) $\land$ (read-coherence) $\land$ (atomicity) $\land$ (PO-RF) \hfill ($\rcmm$)
\end{compactitem}
%We also analyze WeakRC20 model where we drop the (PO-RF) axiom from RC20.

\bparagraph{Relaxed}
Finally, we study the relaxed fragment of $\rcmm$, with only $\MOrlx$ accesses, and thus $\hb = \po$.
\begin{compactitem}
\item (write-coherence) $\land$ (read-coherence) $\land$ (atomicity) $\land$ (PO-RF) \hfill ($\rlxmm$)
\end{compactitem}



\bparagraph{Comparison between memory models}
Considering the possible behaviors allowed by the models discussed above, they can be partially ordered according to their strength as follows:
\[
\inarr{
\scmm \sqsubset \sramm \sqsubset \ramm \sqsubset \set{\wramm, \set{  \rcmm  \sqsubset \rlxmm}}
}
\]
As we go to the right, we obtain a model that allows more behaviors (executions).
In particular, all models are weaker than $\scmm$. 
For the release-acquire models, $\sramm$ is stronger than $\ramm$ and $\ramm$ is stronger than $\wramm$. 
%$\rcmm$ and $\psmm$ are weaker than $\ramm$ as they allow relaxed accesses. 
$\rlxmm$ is weaker than $\ramm$ but incomparable to $\wramm$.
In particular, the lack of synchronization across $\rf$ in $\rlxmm$ makes $\hb$ weaker in $\rlxmm$ compared to $\wramm$.
On the other hand, since $\wramm$ does not require write-coherence, it can also accept behaviors not allowed in $\rlxmm$ because of write-coherence.
Finally, $\rcmm$ can be seen as a combination of $\ramm$ and $\rlxmm$, where fences may retrieve some of the synchronization that goes along relaxed operations.
\cref{fig:mmex} illustrates the differences between these models with small examples.

\input{figures/model_examples}



\bparagraph{The reads-from consistency problem}
An execution $\ex = \tup{\E, \po, \rf, \mo}$ is called \emph{consistent} in a memory model $\M$, written $\ex\models \M$, if it satisfies the axioms of the model.
In many settings, however~\cite{}, one deals with \emph{partial executions} $\expartial=\tup{\E, \po, \rf}$, i.e., where the modification order is missing.
We call $\expartial$ \emph{consistent} in $\M$, written similarly as $\expartial\models \M$, if there exists an $\mo$ such that $\ex\models \M$, where $\ex = \tup{\E, \po, \rf, \mo}$.
Thus the problem of \emph{reads-from consistency checking} (or simply consistency checking, from now on) is to find an $\mo$ that turns $\expartial$ consistent\footnote{Except for $\wramm$, the axioms of which do not involve $\mo$.}
The problem is known to be $\NP$-hard for $\scmm$~\cite{Gibbons:1997}, and in polynomial-time for $\ramm$~\cite{Lahav:2015,Abdulla:2018}.
In this paper we resolve the complexity of consistency checking for all aforementioned memory models, with tight/almost-tight bounds as outlined  in \cref{subsec:contributions}.
The coming sections present these results in detail.
Due to space restrictions, we relegate formal proofs to \cref{sec:app_rf}.






==> contributions_old.tex <==
\bparagraph{Contributions}

In this work we consider the three most common consistency problems for various release-acquire-style memory models.
In each case, the input is a memory model $\MemModel$ and a partial execution $X$ containing the corresponding information, and the task is to decide whether $X$ is consistent with $\MemModel$.
In particular, we focus on the following variants.
\begin{compactenum}
\item \textbf{RV} consistency: $X$ contains the program order $\po$ and the value accessed by each event, but lacks the reads-from map $\rf$.
\item \textbf{RV+MO} consistency: similar to RV, but $X$ also contains the modification order $\mo$.
\item \textbf{RF} consistency: $X$ contains the program order $\po$ and the reads-from map $\rf$, but lacks the modification order $\mo$.
\end{compactenum}

\begin{figure}
\begin{subfigure}[b]{0.2\textwidth}
\[
\inarrC{
X=Y=0;
\\
\inparII{
X=1;
\\ a=X; 
}{
\ X=2;
\\ \ b=X; 
}
}
\]
\caption{$a=2, b=1$}
\end{subfigure}
\hfill\vline\hfill
\begin{subfigure}[b]{0.22\textwidth}
\begin{tikzpicture}[yscale=0.7]
  \node (s) at (0,1)  {$[X=Y=0]$};
  \node (t11) at (-1,0)  {$\wt(X,1)$};
  \node (t12) at (-1,-1.5) {$\rd(X,2)$};
%
  \node (t21) at (1,0) {$\wt(X,2)$};
  \node (t22) at (1,-1.5) {$\rd(X,1)$};
%
  \draw[po] (s) to (t11.north);
  \draw[po] (s) to (t21.north);
  \draw[po] (t11) to node[right]{$\po$} (t12);
  \draw[po] (t21) to node[left]{$\po$} (t22);
%  
%
%   \draw[rf,bend left=0] (t11) to node[below]{$\rf$} (t22);
%   \draw[rf,bend right=0] (t21) to (t12);
% %    
%   \draw[mo,bend left=10] (t11) to  (t21);
%   \draw[mo,bend left=10] (t21) to node[below]{$\mo$} (t11);
\end{tikzpicture}   
\caption{\textbf{RV} trace}
\end{subfigure}
\hfill\vline\hfill
\begin{subfigure}[b]{0.22\textwidth}
\begin{tikzpicture}[yscale=0.7]
  \node (s) at (0,1)  {$[X=Y=0]$};
  \node (t11) at (-1,0)  {$\wt(X,1)$};
  \node (t12) at (-1,-1.5) {$\rd(X,2)$};
%
  \node (t21) at (1,0) {$\wt(X,2)$};
  \node (t22) at (1,-1.5) {$\rd(X,1)$};
%
  \draw[po] (s) to (t11.north);
  \draw[po] (s) to (t21.north);
  \draw[po] (t11) to node[right]{$\po$} (t12);
  \draw[po] (t21) to node[left]{$\po$} (t22);
%  
%
%  \draw[rf,bend left=0] (t11) to node[above]{$\rf$} (t22);
%  \draw[rf,bend right=0] (t21) to node[right]{$\rf$} (t12);
%    
  \draw[mo,bend left=10] (t11) to (t21);
  \draw[mo,bend left=10] (t21) to node[below]{$\mo$} (t11);
\end{tikzpicture}  
\caption{\textbf{RV+MO} trace}
\end{subfigure} 
\hfill\vline\hfill
\begin{subfigure}[b]{0.22\textwidth}
\begin{tikzpicture}[yscale=0.7]
   \node (s) at (0,1)  {$[X=Y=0]$};
  \node (t11) at (-1,0)  {$\wt(X,1)$};
  \node (t12) at (-1,-1.5) {$\rd(X,2)$};
%
  \node (t21) at (1,0) {$\wt(X,2)$};
  \node (t22) at (1,-1.5) {$\rd(X,1)$};
%
  \draw[po] (s) to (t11.north);
  \draw[po] (s) to (t21.north);
  \draw[po] (t11) to node[right]{$\po$} (t12);
  \draw[po] (t21) to node[left]{$\po$} (t22);
%  
%
  \draw[rf,bend left=0] (t11) to node[above]{$\rf$} (t22);
  \draw[rf,bend right=0] (t21) to (t12);
%    
%  \draw[mo,bend left=10] (t11) to node[below]{$\mo$} (t21);
%  \draw[mo,bend right=10] (t22) to (t11);
\end{tikzpicture}
\caption{\textbf{RF} trace}
\end{subfigure}
\caption{Execution $a=2, b=1$: \textbf{RV}, \textbf{RV+MO}, \textbf{RF} traces (merged initial writes and omitted some relation labels). The $\po$, $\rf$, $\mo$ edges denote the respective program-order, reads-from, modification-order relations described in \cref{sec:models}.
}
\end{figure}
\bparagraph{Theoretical contributions.}
We establish a rich landscape of algorithmic and computational complexity of the three main consistency problems (RF, RV+MO, RV)
for various common C11-like memory models.
We refer to \cref{tab:intro} for the full list of our results, while we discuss here some important observations.
\begin{compactenum}
\item We show that the RV consistency problem is hard even for $\NumMemory=1$, for all  considered models.
In fact, hardness arises even on a very restricted setting in which the threads are partitioned into two classes:
a single thread only reads from the shared variable, and all other threads only write to it.
Perhaps surprisingly, $\NumMemory=1$ leads to hardness even for WRA, although it differs from the rest in that  it does not abide to the ``SC-per-location'' principle.

\item RV+MO consistency is known to be $\NP$-hard for SC, even in the basic setting of a single writer thread per variable (thus $\mo$ is subsumed $\po$).
In contrast, we show that for all weak models considered here, the single-writer case admits a nearly linear-time algorithm.
On the other hand, if we lift this restriction and consider an arbitrary $\mo$ in the input, we retrieve hardness.
That being said, the reduction for RA and SRA is somewhat intricate, while WRA follows immediately from the corresponding hardness for RV consistency.

\item Although RF consistency for RA is known to be in polynomial time~\cite{Lahav:2015,Abdulla:2018}
the polynomial involved in these algorithms is at least of quadratic degree.
Here we show that almost all models admit a nearly linear-time algorithm
Perhaps surprisingly, SRA is the only model in which the presence of RMWs makes RF consistency intractable.
At the same time, our $O(\NumThreads\cdot \NumEvents^{\NumThreads})$ bound shows that the hardness depends only on the number of threads $\NumThreads$ (as opposed to the case of RV consistency, where we have hardness on both $\NumThreads$ and $\NumMemory$), 
and thus the problem becomes polynomial-time when $\NumThreads$ is bounded (similarly to SC~\cite{Gibbons1994,Mathur:lics2020}).

\item Finally, we remark that the Relaxed semantics we consider in this work disallow $(\po\cup \rf)^+$ cycles,
to align with RC20~\cite{Margalit:2021}, and as it is followed in most known verification tools for C11.
This requirement is strong enough to make RV consistency for relaxed $\NP$-hard even for $\NumThreads=3$.
In the absence of this restriction, each variable can be processed independently under SC, for which the recent work of \cite{Agarwal:2021} implies a bound of the form $O(\NumThreads^2\cdot n^{\NumThreads+1})$, i.e., polynomial for bounded $\NumThreads$.
\end{compactenum}

\Andreas{Some further relation to the distributed systems problems (@Parosh?)}

\bparagraph{Experiments.}
\Andreas{to be filled.}

\input{tab_intro}

==> executions.tex <==
\subsection{Executions}\label{subsec:executions}

The axiomatic concurrency models are defined with respect to the executions they allow.
Hence, a program can be represented as a set of executions.
In turn, an execution is defined by a set of events that are generated from shared memory accesses or fences, and relations between these events. 

\bparagraph{Events} 
An event is represented by $\tup{\id,\tid,\llab}$ where $\id$, $\tid$, $\llab$ denote a unique identifier, thread identifier, and label of the event. 
A label $\llab=\tup{\op, \ord, \lloc}$ is a tuple where $\op$ denotes the corresponding memory access or fence operation and $\ord$ denotes the 
memory order. 
For memory accesses, $\lloc$ denotes its memory location, while in the case of fences, we have $\lloc = \bottom$. 
In other settings, memory-access events are also labeled by the values they read/write.
As these values are not important for the reads-from consistency problem we study in this paper, we will ignore such values to simplify notation.
%Given an event $\event$, we let $\event.\id$, $\event.\tid$, $\event.\llab$, $\event.\op$, $\event.\ord$, $\event.\lloc$ be the identifier, thread identifier, label, operation, memory order and memory location, respectively.
For an event $\event$, we use notations such as $\event = \wt_o(t, x)$ 
to mean $\event.\op = \wt$, $\event.\ord = o$, $\event.\tid = t$, and $\event.\lloc = x$. When the event's memory order is clear from its context then we write $\wt(t, x)$, and we may simply write $\wt(x)$ to denote a write on $x$ when its thread is not important.

For a set of events $\E$, we will use $\E.locs$ and $\E.tids$ to denote the
set of distinct locations accessed by events in $\E$ and the different threads participating in $\E$. 

%\noindent\textit{Accesses to Events.} 
The set of read, write, atomic update, and fence events are $\R$, $\W$, $\U$ and $\F$ respectively. 
The execution of a load, store, fence access generate an event in $\R$, $\W$, $\F$ respectively. 
As we only deal with executions (as opposed to program source), we use $\U$ to denote a successful read-modify-write operation.
Failed read-modify-write operations simply result to load accesses.
%A successful RMW access generates an $\U$ event and a failed RMW generates an $\R$ event.

We refine the set of events in various ways. 
For instance, we write $\W_{\sqsupseteq \MOrel}$ to denote the set of release or stronger writes and $\R_{\sqsupseteq \MOacq}$ to denote the set of acquire  or stronger reads.
For a set of events $\E$, we use $\locx{\E}$ to denote the subset of events in $\E$
that access memory location $x$. 
The memory locations are initialized at the start of the execution, 
represented by a set of write events. 
%\ucomment{What is the significance of init events being non-atomic?}
% non-atomic init doesn't race. Removing to avoid confusion.


\bparagraph{Notation on relations}
Given a binary relation $S$ over a set of events $\E$, we will use $S(x,y)$ to denote the predicate $(x, y) \in S$.
The reflexive, transitive, reflexive-transitive closures, and inverse relations of $S$ 
are represented by $S^?$, $S^+$, $S^*$, $S^{-1}$ respectively. 
The relation $S$ is acyclic if $S^+$ is irreflexive. Relation $S_\imm$ denotes the immediate relation:  
$S_\imm(x,y) \triangleq S(x,y) \land \nexists z \ S(x,z) \land S(z,y)$. %\ucomment{$S(x,z) \land S(z, y)$}. 
Given two relations $S_1$ and $S_2$, we denote their composition by $S_1;S_2$. 
$[A]$ denotes the identity relation on a set $A$, i.e. 
$[A](x,y) \triangleq x = y \land x \in A$.
For a given memory location $x$, we let $S_x=[\E^x];S;[\E^x]$ be the restriction of $S$ to all events of $\E$ on $x$.


\bparagraph{Candidate Executions and relations}
An execution (also referred to as candidate execution~\cite{Batty:2011} or execution graph~\cite{Lahav:2017}) 
is a tuple $\ex = \tup{\E, \po, \rf, \mo}$  where $\ex.\E$ is a set of events and $\ex.\po$, $\ex.\rf$, $\ex.\mo$ binary relations over $\ex.\E$. 
In particular, relation $\po$ is the \emph{program order}:~it is a partial order and enforcing a total order on events of the same thread. Relation $\rf\colon (\RRMW)\to (\WRMW) $ is the \emph{reads-from function}:~it associates every read/RMW event $\event_1$ to the write/RMW $\event_2=\rf(\event_1)$ that $\event_1$ reads its value from.
Naturally, we require that $\event_1.\lloc=\event_2.\lloc$.
Relation $\mo\subseteq (\WRMW)\times (\WRMW)$ is the \emph{modification order}:~it is the union of modification orders $\mo_x$, where each $\mo_x$ is a total order over $\W^x\cup \U^x$.

We frequently make use of some additional relations derived from $\ex$.
Relation $\fr\subseteq (\RRMW)\times (\WRMW)$ is the \emph{from read relation}, relating every read or RMW event to all the write or RMW events that are $\mo$-after its own writer:
% \begin{align*}
% \fr \triangleq (\rf^{-1};\mo)\setminus [\id]\hfill \tag{from-read}
% \end{align*}
Relation $\sw\subseteq \E_{\sqsupseteq \MOrel}\times \E_{\sqsupseteq \MOacq}$ is the \emph{synchronizes with relation}, relating release and acquire events, for instance, when an acquire read event reads from a release write. 
Fence instructions, and relaxed accesses (in presence of fence instructions)
also participate in $\sw$. 
The precise definition, taken from~\cite{Margalit:2021} (also used in other prior works, such as the \celeventester tool~\cite{Luo:2021}) is:
% \begin{align*}
% \sw \triangleq & \ [\E_{\sqsupseteq \MOrel}];([\F];\po)^?;\rf^+;(\po;[\F])^?;[\E_{\sqsupseteq \MOacq]}] \hfill \tag{synchronizes-with}
% \end{align*}
Relation $\hb$ is the \emph{happens-before relation}, taken as the transitive closure of $\po$ and $\sw$.
We also project $\hb$ to individual locations, denoted as $\hbloc$.
\begin{align*}
\fr \triangleq & \ (\rf^{-1};\mo)\setminus [\id]\hfill \tag{from-read}
\\
\sw \triangleq & \ [\E_{\sqsupseteq \MOrel}];([\F];\po)^?;\rf^+;(\po;[\F])^?;[\E_{\sqsupseteq \MOacq]}] \hfill \tag{synchronizes-with}
\\
\hb \triangleq & \ (\po\cup \sw)^+   \qquad \text{and} \qquad \hbloc \triangleq \ \bigcup_x \hb_x \hfill \tag{happens-before/happens-before-per-location}
\end{align*} 
%\item $\hbloc$ is the \emph{happens-before-per-location relation}, which projects $\hb$ to individual memory locations:
%\begin{align*}
%\hbloc \triangleq & \bigcup_x \hb_x %\tag{happens-before-per-location}
%\end{align*} 
%\item Relation $\poloc$ relates $\po$-related events which access same memory location i.e. $\poloc(a,b) \triangleq \po(a,b) \land a.\lloc = b.\lloc$. 
%Similarly, relation $\hbloc$ denotes $\hb$ relation between same-location events i.e. $\hbloc(a,b) \triangleq \hb(a,b) \land a.\lloc = b.\lloc$. %\ucomment{define $\hb$ first}
%\end{compactitem}

The validity of candidate executions is judged in the context of a memory model.
Axiomatically-defined memory models are defined using sets of axioms, where each axiom prohibits certain executions by posing restrictions on the shape of primary and derived relations.

%\bparagraph{Candidate and consistent executions} 
%An execution (also referred to as candidate execution~\cite{Batty:2011} or execution graph~\cite{Lahav:2017}) 
%is a tuple $\ex = \tup{\E, \po, \rf, \mo}$  where $\ex.\E$ is the set of events and $\ex.\po$, $\ex.\rf$, $\ex.\mo$ are set of $\po$, $\rf$, $\mo$ relations between the events in $\ex.\E$. 
%Pictorially, an execution may be represented as a labeled multigraph over the node set $\ex.\E$, and on which edges capture the various relations between events in $\ex.\E$.
%An execution $\ex$ may or may not represent valid program behavior, 
%which is characterized by the \emph{memory model} $\MemModel$ under which the underlying program executes.
%Formally, the validity of $\ex$ is interpreted within a set of axioms, which pose restrictions on $\po$, $\rf$ and $\mo$.
%If $\ex$ satisfies these constraints, then it is called \emph{consistent} in $\MemModel$,
%denoted $\ex\models \MemModel$.
%In the following, we present the (axiomatic) consistency models we consider in this work.

\begin{figure}
\centering
{\small
\begin{subfigure}{0.45\textwidth}
\begin{compactitem}
%\item $(\poloc \cup \rf \cup \mo \cup \fr)$ is acyclic. \hfill (SC-per-location)
\item $\irr(\mo;\rf^?;\hb^?)$  \hfill (Wcoh) 
\item $\acy(\hb \cup \mo)$ \hfill (strong-Wcoh) 
\item $\irr(\fr;\rf^?;\hb)$ \hfill (Rcoh)
\item $\irr(\hbloc;[\WRMW];\hb;\rf^{-1})$ \hfill (weak-Rcoh)
\\
\item $\irr(\fr;\mo)$ \hfill (atom)
\item $\forall u_1, u_2\in \U, \rf(u_1)\neq \rf(u_2)$ \hfill (weak-atom)
\\
\item $\acy(\po \cup \rf)$ \hfill (PO-RF) 
\end{compactitem}
\end{subfigure}
\hfill\vline\hfill
\begin{subfigure}{0.52\textwidth}
\begin{compactitem}
\item $\ (\po \cup \rf \cup \mo \cup \fr)$ is acyclic. \hfill ($\scmm$)
\\
\item (Wcoh) $\land$ (Rcoh) $\land$ (atomicity) \hfill ($\ramm$)
\item (strong-Wcoh) $\land$ (Rcoh) $\land$ (atomicity) \hfill ($\sramm$)
\item (weak-Rcoh) $\land$ (weak-atomicity) $\land$ (PO-RF) \hfill ($\wramm$)
\\
\item (Wcoh) $\land$ (Rcoh) $\land$ (atomicity) $\land$ (PO-RF) \hfill ($\rcmm$)
\item (Wcoh) $\land$ (Rcoh) $\land$ (atomicity) $\land$ (PO-RF) \hfill ($\rlxmm$)
\end{compactitem}
\end{subfigure}
}
    \caption{Axioms and Models}
    \label{fig:ax:models}
\end{figure}


==> experiments.tex <==
\section{Implementation and Experimental Evaluation}
\label{sec:experiment}

In this section, we present and evaluate an \emph{on-the-fly} algorithm for checking RF consistency in the $\ramm$ fragment. 
The algorithms that were discussed in \crefrange{subsec:rf_wra}{subsec:rf_rlx} constitute \emph{offline} algorithms 
which assume that the set of events on which the RF consistency problem is to be solved is known a priori.
While these algorithms are solving the fundamental consistency checking problems, 
their assumption that the given input events are fixed is not always applicable. 
In particular, certain settings entail continuously extending the execution with new events.
In such settings, the RF consistency problem must be solved incrementally for each observed new read event.
The aforementioned offline algorithms rely on procedures such as cycle detection in a graph, and precomputation of certain relations.
A naive integration of the offline algorithm into such settings would result in the repeated recomputation of these procedures and  lead to a poor performance.
%These procedures enumerate a large segment of all processed events, which can be very large in practice.
%Therefore, such an integration would lead to a poor performance and 
%Alternative on-the-fly algorithms, which can perform incremental consistency checks, are better suited for these settings.
Our focus in this section is to present an efficient on-the-fly algorithm which solves the incremental RF consistency problem.
One such setting in which the RF consistency problem is needed to be solved incrementally is in dynamic analysis tools such as \celeventester~\cite{Luo:2021}. % which is a state-of-the-art concurrency testing tool. 
We implemented the proposed algorithm inside the \celeventester framework and performed a comparison with the original implementation. 
Our experimental evaluation based on the benchmarks found in the recent literature demonstrates that the proposed algorithm is able to provide a speedup up to $\maxspeedup \times$ and $\avgspeedup \times$ on average. %compared to the original \celeventester implementation.
In the remainder of this section, we describe the proposed algorithm in detail (\cref{sec:on-the-fly-algo}), contrast the original \celeventester implementation with the proposed algorithm (\cref{sec:compare-c11tester}), and report on our experimental evaluation (\cref{sec:experiment-standard}).  

\subsection{On-the-fly Algorithm}
\label{sec:on-the-fly-algo}
\input{algorithms/algo-ra-rf-on-the-fly}                                                         
%In this section we describe our on-the-fly algorithm for solving RF consistency problem in the $\ramm$ fragment. 
Let $\expartial = \tup{\E, \po, \rf}$ be a partial and incomplete execution for which there exists an $\co$ such that $\expartial$ is consistent in $\ramm$. 
The task is to determine if there exists an $\co'$ such that the execution $\expartial' = \tup{\E', \po', \rf'}$ is consistent in $\ramm$ where $\E \subset \E'$, $ \po \subseteq \po'$ and $\rf \subseteq \rf'$ are obtained after adding a new event into the execution.  
The pseudocode of the proposed algorithm solving this task is shown in \cref{algo:ra-rf-on-the-fly}~\footnote{For ease of presentation, we assume that the number of threads in the program is fixed and known a priori.}.
When a new read or write event is observed, the functions $\rdhandler$ and $\wthandler$ are called, respectively. 
RMW events are handled by first calling $\rdhandler$ followed by $\wthandler$.
%After the algorithm processes an event it stores the event's corresponding $\hb$ relation in the $\HB$ clock. 
\cref{algo:ra-rf-on-the-fly} cannot utilize the helper functions $\getHBTS$ and $\getLRWB$ as the previous algorithms. 
Instead, it maintains the same information obtained from these functions on-the-fly (Lines \ref{line:ra-otf-hb}, \ref{line:ra-otf-getlw}, \ref{line:ra-otf-trans-closure-2}, \ref{line:ra-otf-write-hb-update}-\ref{line:ra-otf-write-glw}).
Overall, \cref{algo:ra-rf-on-the-fly} has a similar working mechanism as \cref{algo:rf-consistency-rc20}. 
It infers a necessary and sufficient set of partial modification orderings, for which
there are guaranteed total extensions that are compliant with the $\ramm$ model.
When a new event is observed, \cref{algo:ra-rf-on-the-fly} aims to infer new $\mo$ edges based on \cref{lem:read_coherence} and \cref{lem:RC20-RF-Consistency-Chain-Rule} and then performs certain checks to ensure that consistency is maintained.
%Intuitively, the $\HBMO$ clock of a given write event $w$ captures the incoming $\mo$ edges to $w$.
%The algorithm stores the $\hb$ and $(\hb \cup \bigcup_{x \in \E.locs}\mo_{\partialtext, x})$ relations per event in the $\HB$ and $\HBMO$ \todo{incoming $\mo$ edge information} 
%The clock $\Hh$ is used for maintaining the local $\hb$ clocks per thread. 
%inferring new $\mo$ edges.
%We refer to this process is as saturation.
%In the $\ramm$ fragment, 
%Lines are similar to 
%After this step, .
%If $w_\rf$ is an RMW event then the propagation is conducted from the head of the RMW chain.
%if the new inferred edges leads to a cycle in the $(\hb \cup \mo_{\partialtext, x\in\E.locs})$ relation.
%The algorithm employs an elaborate procedure for performing the cycle detection to enable efficient analysis. 
Below we describe the procedure that the algorithm performs for each  new event it observes.
\begin{compactitem}
	\item{ 		
	For a new read event $\event = \rd(t, x)$ (or $\event = \ud(t, x)$) with $w_{\rf} = \rf(\event)$, in the first part of the procedure (\crefrange{line:ra-otf-hb}{line:trans-closure-end}) the algorithm performs certain checks (Lines \ref{line:ra-otf-first-check-begin},  \ref{line:ra-otf-third-check-begin2}, \ref{line:ra-otf-trans-closure-3}) 
	to ensure that extending the execution with $\event$ results in a consistent execution.
	These checks are performed by means of an acyclicity check and they ensure 
	that the write coherence and atomicity axioms are not violated.
	A core component of the algorithm is the $\HBMO$ clocks, which are essential for performing efficient acyclicity checks.
	Each write event in the execution has an associated $\HBMO$ clock which stores the 
	relation $(\hb \cup \mo_{\partialtext, x\in\E.locs})$.
	RMW events in the same chain are represented with a single $\HBMO$ clock.
	%We remark that in the pseudocode of \cref{algo:ra-rf-on-the-fly}, it is implicitly assumed that $\HBMO[\event]$ points to the $\HBMO[\TC[\event]]$ if $\event.\op = \ud$. 
	Intuitively, $\HBMO$ clock of a write event $w$ captures the incoming $\mo$ edges to $w$ from the writes in the other threads. 
	The acylicity check is performed by checking that write events that are determined by the principles outlined in \cref{lem:read_coherence} and \cref{lem:RC20-RF-Consistency-Chain-Rule} do not have an incoming $\mo$ edge from $w_\rf$.
	An important feature of \cref{algo:ra-rf-on-the-fly} is that to optimize for performance, it does not keep the $\HBMO$ clocks transitively closed.
	Due to this reason, the algorithm may fail to reject an inconsistent execution in the first checks that it performs  (\crefrange{line:ra-otf-hb}{line:ra-otf-check-end}). 
	In \crefrange{line:trans-closure-init}{line:trans-closure-end}, a transitive closure procedure is conducted and the acyclicity is checked again (\cref{line:ra-otf-trans-closure-3}).
	If this step is passed, then the algorithm updates the state of the execution (\crefrange{line:ra-otf-update-hbmo}{line:ra-otf-last}) and declares that the execution is consistent.
	%Even though $\HBMO$ clocks are not kept transitively closed, 
	While the algorithm is updating the state of the execution, it propagates the new inferred $\mo$ edges on the $w_\rf$ into the writes that are $\po$ ordered after $\TC[w_\rf]$ (\cref{line:ra-otf-po-prop}). 
	%If $w_\rf$ is an RMW event then the propagation is performed on the $\TC[w_\rf]$ (\cref{line:ra-otf-po-prop-end}).
	%In \crefrange{line:ra-otf-po-prop-start}{line:ra-otf-po-prop-end} the algorithm propagates the new inferred $\mo$ edges into the writes that are $\po$ ordered after $w_\rf$.
%	infers new $\mo$ edges and decides if the new edges would results in a cycle in the $(\hb \cup \bigcup_{x \in \E.locs}\mo_{\partialtext, x})$ relation. 
%	The algorithm initially iterates over all threads and fetches the last write event $w$ performed by each thread on location $x$ which is $\hb$-ordered before $\event$ (\cref{line:ra-otf-getlw}). 
%	This procedure is conducted by utilizing the function $\getLW$ (see \cref{algo:ra-rf-on-the-fly-helper}). 
	%\todo{write this part} Note that in previous sections this function was precomputed whereas here this function is computed on-the-fly.  
%	After fetching such a write event $w$, the algorithm follows a certain procedure to either infer the $\mo$ edge $(w, w_\rf)$ (unless $w = w_\rf$) or declare that the execution is inconsistent.
%	The algorithm starts by performing a number of checks to deduce if the execution is inconsistent (\crefrange{line:ra-otf-first-check-begin}{line:ra-otf-third-check-end}). 
%	The first check (\crefrange{line:ra-otf-first-check-begin}{line:ra-otf-first-check-end}) ensures that if $w$ and $w_{\rf}$ are in the same RMW chain then $w_{\rf}$ is not $\hb$ ordered before $w$.
	%CFL as this would imply that the $\mo$ edge $(w_\rf, w)$ already exists and inferring the $\mo$ edge $(w, w_\rf)$ would lead to an inconsistent execution. 
%	If $w$ and $w_\rf$ are in the same RMW chain but $w$ is $\hb$ ordered before $w_\rf$ then the algorithm disregards this $w$ and continues with the write event in the next thread (\cref{line:ra-otf-first-check-end}). 
%	The case where $w$ and $w_\rf$ are in the same RMW chain requires this special treatment as the algorithm maintains a single $\HBMO$ clock for all the events in an RMW chain. 
%	This aspect of the algorithm is further explained in \cref{sec:efficient-rmw-handling}.
%	The second check (\crefrange{line:ra-otf-second-check-begin}{line:ra-otf-second-check-end}) ensures that the $\mo$ edge $(w_\rf, w)$ does not exist.
%	The third check (\crefrange{line:ra-otf-third-check-begin}{line:ra-otf-third-check-end}) ensures that if $w_\rf$ is an RMW event then the $\mo$ edge ($w_\rf.\chainhead$, $w$) does not exists.
%	If $w$ passes through all the above checks then the algorithm joins the $\HBMO$ clock of $w$ with an auxiliary clock $\PHBMO$ which keeps the maximal $\HBMO$ clocks across all threads.
%	Intuitively, $\PHBMO$ keeps all new incoming $\mo$ edges into $w_\rf$, 
%	and it will later be joined with the $\HBMO$ clock of $w_\rf$ unless the execution turns out to be inconsistent.
%	One of the main features of \cref{algo:ra-rf-on-the-fly} is that, for efficiency reasons, the $\HBMO$ clocks of write events are not kept transitively closed. 
%	Therefore, in \crefrange{line:trans-closure-init}{line:trans-closure-end} the algorithm performs a transitive closure procedure.
%	The algorithm iterates over the set $L$ which is initialized with the set of all threads.
%	For each thread $t'$ in $L$, it checks if $\event$ is $\hb$ aware of the corresponding write event of $t'$ in $\PHBMO$ (\cref{line:ra-otf-trans-closure-1}). 
%	If this is the case then the algorithm does not compute the transitive closure for the write event of the thread $t'$.
%	The reason for this is that if $\event$ is $\hb$ aware of a write then this event must have already been considered in the above loop (\crefrange{line:ra-otf-first-loop-start}{line:ra-otf-check-end}). 
%	If $\event$ is not $\hb$ aware of the event of $t'$ in $\PHBMO$ then the algorithm proceeds to compute the transitive closure of the corresponding write event.
%	The algorithm fetches the last write event $w''$ on location $x$ executed by thread $t'$ which is ordered before the $t'$-th entry in $\PHBMO$ clock (\cref{line:ra-otf-trans-closure-2}).
%	It then checks if the $\mo$ edge ($w_\rf, w''$) exists and if so declares the execution inconsistent (\crefrange{line:ra-otf-trans-closure-3}{line:ra-otf-trans-closure-4}).
%	Otherwise, $\PHBMO$ clock is joined with the $\HBMO$ clock of $w''$ by calling the function $\joinchangedindex$ (see \cref{algo:ra-rf-on-the-fly-helper}).
%	This function is utilized to keep track of the entries that are changed during the join operation.
%	The changed entries are added to the set $changedIndexes$.
%	In \cref{line:trans-closure-end} $L$ is set to $changedIndexes$ and $changedIndexes$ is set to an empty set. 
%	This loop is iterated until $changedIdexes$ (and consequently $L$) remains as an empty set at the end of the inner loop.
%	This intuitively implies all required $\mo$ edges are inferred and the execution was found to be consistent.
%	In \cref{line:ra-otf-update-hbmo} the algorithm updates the $\HBMO$ clock of $w_\rf$ with the new inferred $\mo$ edges and in \cref{line:ra-otf-update-hb} $\HB$ clock of $\event$ is updated.
%	In \crefrange{line:ra-otf-po-prop-start}{line:ra-otf-po-prop-end} the algorithm propagates the new inferred $\mo$ edges into the writes that are $\po$ ordered after $w_\rf$.
%	If $w_\rf$ is an RMW event then the propagation is conducted from the head of the RMW chain.
%	%This results in only partially inferring new $\mo$ edges.
%	This results in $\HBMO$ clocks of the write events to be not transitively closed.
%	This aspect of the algorithm is further explained in \cref{sec:no-prop-across-threads}.
	}
	\item{
	For a new write event $\event = \wt(t, x)$ (or $\event = \ud(t, x)$), the main goal of the procedure is to initialize or update the $\HBMO$ clock of $\event$.
	%observe that extending a consistent execution with $\event$ cannot lead to making the execution inconsistent.
	%Therefore, the algorithm performs a simpler procedure for handling new write events.
	In particular, the algorithm first fetches the write event $w$ which corresponds to the last executed write event in thread $t$ on location $x$.
	The algorithm then joins $\HBMO[\TC[\event]]$ with $\HBMO[w]$ and $\HB[\event]$ (\cref{line:ra-otf-write-rmw-hbmo}) and propagates the new inferred $\mo$ edges into the writes that are $\po$ ordered after $\TC[\event]$.
	Note that the latter step is only relevant for the write events that are associated with an RMW chain. 
	%If $\event$ is the write part of an RMW event then, as the algorithm maintains a single $\HBMO$ clock for all the events in an RMW chain, it joins $\HBMO[\TC[\event]]$ with $\HBMO[w]$ and $\HB[\event]$ (\cref{line:ra-otf-write-rmw-hbmo})
	%and  (\cref{line:ra-otf-write-rmw-hbmo-po}).
	%Otherwise, the algorithm initializes $\HBMO[\event]$ with the join of $\HBMO[w]$ and $\HB[\event]$ (\cref{line:ra-otf-write-hbmo}).
	%If a new write event is observed. Normally, one would need to find all the hb paths similar to the case of observing a new read event. However, . Therefore, the algorithm does not attempt to find all the $\hb$ paths. 
	%The algorithm then infers the $\mo$ edge $(w, w_\rf)$, unless $w = w_\rf$ (\cref{line:ra-otf-check-end}).
	%Lines corresponding to the possible $\mo$ edges to be inferred.  
	%On line $\PHBMO$ will be joined with the $\HBMO$ clock of $w_{\rf}$ and the new $\mo$ edges will be inferred. 
	}
\end{compactitem}

The working mechanism of the \cref{algo:ra-rf-on-the-fly} described above incorporates certain special features. 
The main purpose of introducing such features is to enable inferring fewer explicit $\mo$ edges to gain better performance. 
Below we provide a discussion on each such feature of \cref{algo:ra-rf-on-the-fly}.
%Below we first outline a summary of the main features of the proposed algorithm and then provide a more detailed discussion of each feature.
%\begin{enumerate}
%	\item The incoming $\mo$ edges into the RMW events that are in the same RMW chain are compactly represented as a single clock. \itmlabel{rmw-single-clock}
%	\item New $\mo$ edges resulting from RMW atomicity axiom are partially inferred. \itmlabel{rmw-partial-infer}
%	\item Partial saturation is performed for processing new read events. \itmlabel{read-partial-saturation}
%	\item No saturation is performed for processing new write events. \itmlabel{write-no-saturation} 
%\end{enumerate}
%
%The main purpose of introducing the above features is to enable inferring fewer explicit $\mo$ edges to gain better performance. 
%The features (\itmref{rmw-single-clock}) and (\itmref{rmw-partial-infer}) are explained in \cref{sec:efficient-rmw-handling} and the features (\itmref{read-partial-saturation}) and (\itmref{write-no-saturation}) are explained in \cref{sec:no-saturation-write} and \cref{sec:no-prop-across-threads}, respectively. 
%Furthermore, one side feature of the proposed algorithm is that
%it does not require to perform any rollback in case the current execution turns out to be inconsistent. 
%In particular, if the current selection of $\rf$ leads to an inconsistent execution, then in practice a new $\rf$ will be chosen and the RF consistency checking procedure is repeated.
%Therefore, special care may be required to not contaminate the state of the algorithm in case the current choice of $\rf$ leads to an inconsistent execution~\cite{Luo:2021}. 
%The proposed algorithm straightforwardly maintains all the relevant information for processing a new event in auxiliary data structures until it is known that the execution is consistent.

\subsubsection{Efficient Handling of RMW Events}
\label{sec:efficient-rmw-handling}
%Outgoing and incoming $\mo$ edges from and into the events in an RMW chain entail certain new $\mo$ edges to be inferred, as depicted in \crefrange{subfig:rmw-infer-1}{subfig:rmw-infer-2} where \circled{1} denotes the newly added edge and \circled{2} denotes the inferred edge.
Atomicity axiom requires inferring certain $\mo$ edges as depicted in \crefrange{subfig:rmw-infer-1}{subfig:rmw-infer-2}, where \circled{1} denotes the newly added edge and \circled{2} denotes the inferred edge.
\cref{algo:ra-rf-on-the-fly} maintains a single $\HBMO$ clock for all the events in an RMW chain (\cref{line:ra-otf-write-rmw-hbmo}).
%This corresponds to representing the incoming $\mo$ edges to all the events in an RMW chain as a single clock.
Whenever the corresponding $\HBMO$ clock of an RMW event is updated, this naturally results in all the events in this chain to become aware of this update.
Therefore, \cref{algo:ra-rf-on-the-fly} effortlessly infers the type of edges depicted in \cref{subfig:rmw-infer-1}. 
Adding a new outgoing $\mo$ edge from an RMW event also requires inferring certain edges, as depicted in \cref{subfig:rmw-infer-2}.
However, \cref{algo:ra-rf-on-the-fly} does not explicitly infer such edges. 
The reason why \cref{algo:ra-rf-on-the-fly} still maintains correctness can be illustrated as follows. 
Consider the scenario depicted in \cref{subfig:rmw-inconsistent-exec} and assume that initially the edge \circled{1} is added. 
\cref{algo:ra-rf-on-the-fly} does not infer the edge \circled{2}, while ensuring that if later such an edge like \circled{3} is added then it is able to discover the inconsistency of the execution.  
This follows from that if the edge \circled{3} is added then the algorithm would infer the edge \circled{4} (as depicted in \cref{subfig:rmw-infer-1}). 
This would allow it to discover the inconsistency through the cycle formed by the edges \circled{1} and \circled{4}.
%Note that representing all the events in an RMW chain as a single $\HBMO$ clock does not necessarily assist in inferring the edges depicted in \cref{subfig:rmw-infer-2}.
%For instance, in \cref{subfig:rmw-inconsistent-exec} if the edge \circled{1} is added after the RMW event is executed then adding the edge \circled{1} naturally corresponds to adding \circled{2} at the same time as these events are represented as a single $\HBMO$ clock.
%However, this is not the case if the RMW event is executed after the edge \circled{1} is added. 
\input{figures/rmw_on_the_fly_handling}


\subsubsection{Partial Saturation for New Read Events}
\label{sec:no-prop-across-threads}
Consider the scenario depicted in \cref{subfig:ra-rf-otf-po-prop} where the event $\event_5$ is the last processed event and $\event_6$ has not been processed yet.
%When \cref{algo:ra-rf-on-the-fly} processes a new read event $\event = \rd(t, x)$ (or $\event = \ud(t, x)$) with $\event_2 = \rf(e)$, it infers the new $\mo$ edge ($\event_1, \event_2$) where $\event_1 = \wt(t_1, x)$ is the last write event in the thread $t_1$ that is $\hb$ ordered before $\event$.
The $\mo$ edge ($\event_1, \event_2$) has been inferred after processing $\event_5$. 
Observe that due to the existing $\mo$ edges ($\event_2, \event_3$) and ($\event_2, \event_4$), 
a naive version of \cref{algo:ra-rf-on-the-fly} would compute the transitive closure and update the $\HBMO$ clocks of both $\event_3$ and $\event_4$ accordingly.
However, \cref{algo:ra-rf-on-the-fly} updates $\HBMO[\event_3]$ but $\HBMO[\event_4]$ remains unchanged.
In particular, \cref{algo:ra-rf-on-the-fly} maintains the following invariant.
\begin{restatable}{lemma}{RA-OTF-PO-PROP}
	\label{lem:ra-otf-po-prop}
	Let $\event_1 = \wt(t, x)$ and $\event_2 = \wt(t, x)$ be the events processed by \cref{algo:ra-rf-on-the-fly}. Then, $\HB[\event_1] \sqsubseteq \HB[\event_2] \implies \HBMO[\event_1] \sqsubseteq \HBMO[\event_2]$.  
\end{restatable}
Intuitively, whenever a write event $w$ has new incoming $\mo$ edges, \cref{algo:ra-rf-on-the-fly} only propagates this information to a write event $w'$ if $(w, w') \in \po$.
%This implies that \cref{lem:ra-otf-po-prop} does not hold if the events are in different threads.
%For this reason, \cref{algo:ra-rf-on-the-fly} does not infer the edge ($\event_1, \event_5$) explicitly as $\event_2.\tid \neq \event_5.\tid$.
%This results in that the $\HBMO$ clocks of write events are not necessarily transitively closed.
The reason as to why this preserves correctness of the algorithm can be illustrated as follows. 
Consider the example in \cref{subfig:ra-rf-otf-po-prop} again and assume that algorithm is now processing a new event $\event_6$ with $\event_1 = \rf(\event_6)$.
Observe that this would lead to an inconsistent execution as  $(\event_1, \event_4) \in \mo$. 
%which are the last write events on location $x$ that are $\hb$ ordered before $\event'$ on threads $t_3$ and $t_4$, respectively.
However, event $\event_4$ is in fact not aware of the incoming $\mo$ edge from $\event_1$ as the algorithm did not update $\HBMO[\event_4]$.
Nevertheless, event $\event_2$ or some $\po$ successor of it (due to \cref{lem:ra-otf-po-prop}) is aware of the incoming $\mo$ edge from $\event_1$.
If $(\event_2, \event_6) \in \hb$ then 
%within the first loop of the $\rdhandler$ function (\crefrange{line:ra-otf-hb}{line:ra-otf-check-end}) 
the algorithm will fetch $\event_2$ (or a $\po$ successor) in \cref{line:ra-otf-getlw} and it will be able to discover the inconsistency in the following checks.
If $(\event_2, \event_6) \not \in \hb$ then the inconsistency will be discovered during the transitive closure procedure on the $\HBMO$ clock of $\event_4$  (\crefrange{line:trans-closure-init}{line:trans-closure-end}).
%The algorithm will be able to discover the inconsistency when it performs the transitive closure on the $\HBMO$ clock of $\event_4$.
%and the algorithm discovers that the execution is inconsistent through the information that is present in the $\HBMO$ clock of $\event_2$.
%Moreover, due to \cref{lem:ra-otf-po-prop}, if the last write event in thread $t_3$ on location $x$ that is $\hb$ ordered before $\event$ is a different write event than $\event_2$ (e.g. $\event_3$) then the algorithm would still be able to discover that the execution is inconsistent as all the write events that are $\po$ ordered after $\event_2$ will be aware of $\event_1$.
Note that \cref{lem:ra-otf-po-prop} does not hold if the preceding event is an RMW event. 
%As discussed in \cref{sec:efficient-rmw-handling}, if an RMW event has a new incoming $\mo$ edge then this edge must be added to all the events in the RMW chain. 
%If \cref{algo:ra-rf-on-the-fly} aims to keep the invariant in \cref{lem:ra-otf-po-prop} for RMW events as well then this would require performing propagation to all write events that are $\po$ ordered after any of the events in the RMW chain.
Whenever the $\HBMO$ clock of an event $\event$ in an RMW chain is updated, \cref{algo:ra-rf-on-the-fly} only
propagates this information to a write event $w'$ if $(\TC[\event], w') \in \po$ (\cref{line:ra-otf-po-prop}).
This preserves correctness of the algorithm due to the following observation.
\begin{restatable}{corollary}{RA-OTF-RMW-PROP}
	\label{cor:ra-otf-rmw-prop}
	Let $\event_1 = \ud(t, x)$ and $\event_2 = \rd(t', x) \lor \ud (t', x)$ be the events processed by \cref{algo:ra-rf-on-the-fly}. Then, $\HB[\event_1] \sqsubseteq \HB[\event_2] \implies \HB[\TC[\event_1]] \sqsubseteq \HB[\event_2]$.  
\end{restatable}

For an intuition, consider the scenario depicted in \cref{subfig:ra-rf-otf-rmw-prop}.
Assume that the $\mo$ edge $(\event_3, \event_2)$ is added, which results in an update on $\HBMO[\TC[\event_2]]$.
\cref{algo:ra-rf-on-the-fly} propagates these changes into $\HBMO[\event_4]$ but $\HBMO[\event_5]$ remains unchanged.
%However, this information is not propagated to the writes that are $\po$ ordered after $\event_2$.
Assume now that the algorithm is processing a new event $\event_6 = \rd(t_4, x)$ with $\event_3 = \rf(\event)$. 
Observe that this would lead to an inconsistent execution as both $(\event_3, \event_4)$, $(\event_3, \event_5) \in \mo$.
%ordered before both $\event_4$ and $\event_5$ which are the last write events on location $x$ that are $\hb$ ordered before $\event$ on threads $t_1$ and $t_2$, respectively.
Notice that the write event $\event_5$ is in fact not aware of the incoming $\mo$ edge from $\event_3$ as $\HBMO[\event_5]$ was not updated in the last step.
However, $\event_4$ is aware of this edge and the algorithm discovers the inconsistency through $\event_4$.
Note that due to \cref{cor:ra-otf-rmw-prop}, $(\event_2, \event_6) \in \hb \implies (\event_1, \event_6) \in \hb$ will always hold.
Moreover, if an event like $\event_4$ is present such that  $(\event_1, \event_4) \in \po$ and $(\event_4, \event_6) \in \hb$ then due to \cref{lem:ra-otf-po-prop}, $\HBMO[\event_1] \sqsubseteq \HBMO[\event_4]$ will hold. 
%Hence, the algorithm will always be able to discover that such an execution is inconsistent.
\input{figures/ra_rf_on_the_fly_po_prop}

\subsubsection{No Saturation for New Write Events}
\label{sec:no-saturation-write}
%If we only do saturation when we see a read event then this can also lead to more flexibility to the underlying fuzzing algorithm.
%That is, we spend only minimal amount of time for processing writes.
%Moreover, if the underlying fuzzer decides to fuzz a small number of reads than all reads overall we would obtain a very efficient procedure.  

%Observe that in the $\ramm$ fragment read events can only read from preceding write events. 
%Observe that a new write event can only have incoming $\mo$ edges and not outgoing $\mo$ edges. 
Observe that adding a new write event cannot result in making a consistent execution inconsistent. 
%A consequence of this is that one can directly deem that the execution is consistent after adding a new write event into the execution %$\event = \wt(t, x)$  without performing saturation. 
\cref{algo:ra-rf-on-the-fly} utilizes this fact and only employs a minimal effort to initialize or update the $\HBMO$ clock of $\event$.
In particular, in this process it only fetches the $\HBMO$ clock of the latest thread local predecessor write event of $\event$ on location $x$.
%In contrast, if the algorithm was aiming to keep the $\HBMO$ clocks transitively closed, then for each new observed write event $\event = \wt(t, x)$, it would be required to iterate over all the threads and fetch the latest write event on location $x$ that is $\hb$ ordered before $\event$, similar to the case of handling read events. %CML
This procedure speeds up the process of handling write events. 
However, this also implies that $\HBMO[\event]$ do not possess all the information and it is one of the reasons the algorithm is required to perform the transitive closure procedure in the handling of read events (\crefrange{line:trans-closure-init}{line:trans-closure-end}).
%The reason behind \cref{algo:ra-rf-on-the-fly} favors not performing saturation for the new write events is that the new information obtained from the saturation process may not necessarily be always utilized.  
%In particular, this information is needed when a write event is the latest $\hb$ predecessor of a new read event in some given thread and location.
%If a write event never appears in this position then performing full saturation on this write event has no direct utilization.
%Moreover, the latest $\hb$ predecessors of a new read event may have incoming $\mo$ edges from different write events in a particular thread. 
%\cref{algo:ra-rf-on-the-fly} joins the $\HBMO$ clocks of all the latest $\hb$ predecessors of a read event into an auxiliary clock (\cref{line:ra-otf-check-end}) which is then used as a basis for computing the transitive closure. 
%Hence, this results in only performing full saturation on the latest writes in each thread (\crefrange{line:trans-closure-init}{line:trans-closure-end}) and disregarding the intermediate writes.
%This can reduce the effort to perform saturation. 
%consider two write events $w_1 = \wt(t_1, x)$ and $w_2 = \wt(t_2, x)$ that are the latest $\hb$ predecessors of a new read event.  if while other write events may already be aware of a later write 
%Delaying to perform the  full saturation on the latest write per thread.
%For these reasons, \cref{algo:ra-rf-on-the-fly} refrains from performing saturation when it observes a new write event.
%However, if one aims to keep the $(\hb \cup \bigcup_{x \in \E.locs}\mo_{\partialtext, x})$ relation transitively closed then saturation must be performed.
 



\subsection{Comparison with the C11Tester Algorithm}
\label{sec:compare-c11tester}
\celeventester is a tool for concurrency testing C11 programs.
The main design goal of \celeventester is to find data races in C/C++ programs that utilize atomics.
\celeventester performs controlled execution of C11 programs and aims to explore different program behaviors by fuzzing the thread scheduler as well as the $\rf$ relation.
We concentrate on the procedure performed for fuzzing the $\rf$ relation,
which can benefit from an efficient on-the-fly algorithm that solves the RF consistency problem. 
In particular, fuzzing the $\rf$ relation entails that whenever a new read event $r$ is observed, 
first a write event $w$ is chosen with respect to a certain strategy and $\rf$ is updated such that $w = \rf(r)$. 
Then, it is checked if this particular choice of $\rf$ results in a consistent execution.
In case an inconsistent execution is obtained then an alternative write event is chosen and the procedure is repeated.      
This process is conducted for all observed read operations. 
This results in \celeventester to continually solve the RF consistency problem for each observed read event. 
%\celeventester provides a framework in which the $\rf$ relation and the thread scheduling is resolved based on a fuzzing procedure.
%This enables \celeventester to examine different paths in the program and possibly discover more bugs.
%This setting requires \celeventester to continuously solve the RF consistency problem.
Similar to \cref{algo:ra-rf-on-the-fly}, \celeventester infers new $\mo$ edges with each observed new event and 
then it checks whether the newly inferred $\mo$ edges results in a consistent execution.
To this end, \celeventester utilizes a data structure called $\mo$-graph which maintains the $\mo$ relation. 
The notion of $\mo$-graph is analogous to $\HBMO$ clocks in \cref{algo:ra-rf-on-the-fly}.
%If the newly inferred edges does not result in a cycle in the $\mo$-graph then the execution is deemed to be consistent.
The main differences between \cref{algo:ra-rf-on-the-fly} and \celeventester are as follows.
First, \celeventester keeps the $\mo$-graph transitively closed.
This is in direct contrast with the \cref{algo:ra-rf-on-the-fly} as 
the $\HBMO$ clocks are not kept transitively closed. 
%This aspect of \cref{algo:ra-rf-on-the-fly} is further discussed in \cref{sec:no-prop-across-threads} and \cref{sec:no-saturation-write}.
Second, \celeventester and \cref{algo:ra-rf-on-the-fly} differ in their way of handling RMW events.
In \celeventester RMW events in the same chain are represented as different nodes in the $\mo$-graph, as opposed to the compact representation of these events in \cref{algo:ra-rf-on-the-fly}.
Third, whenever an outgoing edge is needed to be added from an RMW event, \celeventester has to follow the RMW chain of this event and add the edge from the end of the chain. 
Such edges are not explicitly added in \cref{algo:ra-rf-on-the-fly}.
%These aspects \cref{algo:ra-rf-on-the-fly} are further discussed in \cref{sec:no-prop-across-threads}.
%\cref{sec:experiment-synthetic} discusses certain synthetic benchmarks which provides more insight on the differences between \celeventester and \cref{algo:ra-rf-on-the-fly}.



\subsection{Experimental Evaluation}
\label{sec:experiment-standard}

In this section we report on an experimental evaluation of \cref{algo:ra-rf-on-the-fly}.
The main goal of this evaluation is to assess the practical benefits of \cref{algo:ra-rf-on-the-fly} over the state-of-the-art \celeventester tool for performing on-the-fly RF consistency checking in C11 programs.
We implemented \cref{algo:ra-rf-on-the-fly} inside the \celeventester tool with minimal modifications on the original tool environment.
We performed our evaluation in a setting where \cref{algo:ra-rf-on-the-fly} runs alongside with the \celeventester and both techniques observe the same execution and solve the same RF consistency queries. 
The time taken to perform saturation is used as the metric to compare the two techniques. 
%We evaluated evaluate the proposed algorithm. 
%\begin{itemize}
%\item{
%	\expsetone: In this setting \cref{algo:ra-rf-on-the-fly} runs alongside with the \celeventester and both techniques observe the same execution and solve the same RF consistency queries. 
%	Time to perform saturation is used as the metric to compare the two techniques. 
%	}
%\item{
%	\expsettwo: In this setting \cref{algo:ra-rf-on-the-fly} is implemented as a separate tool and compared against the original  implementation of \celeventester.
%	Overall analysis time is used to compare the two techniques.
%	}
%\end{itemize}
%Experimenting in both settings \expsetone and \expsettwo contribute in performing a more thorough evaluation of the proposed algorithm.
Performing evaluation in the setting \expsetone ensures that both techniques observe the same input. 
Note that in case the techniques are employed independently then even in the analysis of the same program differences could arise due to the fact that the $\rf$ relation might be resolved differently.
This would result in techniques to solve different RF consistency queries.
Our evaluation setting prevents this issue and fosters a more suitable environment for the direct comparison of the techniques.   
%Whereas \expsettwo corresponds to the intended usage setting of the tools. 
%Moreover, experimenting in both \expsetone and \expsettwo aids in more clearly understanding the effect of saturation time into the overall execution time.
The benchmarks used to perform the evaluation consists of the benchmarks used in recent literature~\cite{Abdulla:2018, Luo:2021, Lidbury:2017, NorrisDemsky:2013, Kokologiannakis:cav:2021}.
In particular, we used the CDSChecker benchmarks from \cite{NorrisDemsky:2013}, $8$ benchmarks used in \cite{Abdulla:2018} the application benchmarks  Silo, GDAX, Mabain, Iris, and JSBench used in \cite{Luo:2021} and $9$ data structure benchmarks used in \cite{Kokologiannakis:cav:2021}. 
This resulted in a total of $33$ benchmarks.
Certain benchmarks were scaled (e.g. by increasing the number of threads or loop counters) in order to obtain large executions that enable a meaningful comparison of the techniques.
The experiments were conducted on a laptop running Ubuntu 20.04 LTS with 1.8GHz Intel Core i7 processor and 16GB RAM.
All experiments were repeated $10$ times and the average results are reported.
We remark that the obtained benchmarks contain accesses outside the scope of the $\ramm$ model.
In such cases we converted those accesses to an applicable access mode in the $\ramm$.
That is, $\MOrlx$ and $\MOsc$ accesses are converted into $\MOacq$ and $\MOrel$ accesses.
%Moreover, as discussed 
The results of the experimental evaluation are displayed in~\cref{tab:expr-results-2}.
We observe that \cref{algo:ra-rf-on-the-fly} is able to provide an average speedup of $4.82$..
The results also indicate that \cref{algo:ra-rf-on-the-fly} displays either a comparable performance with \celeventester or it outperforms \celeventester in all the benchmarks.
%In table the results of the evaluation performed on the synthetic benchmarks are displayed.
%The results indicate that.
%\input{tab_experiments}
\input{tab-experiments-2-old}
\input{figures/scalability}


==> helpers-old.tex <==
%!TEX root=./main.tex

\section{Auxiliary Functions and Observations}\label{sec:helper_functions}

Several of our consistency-checking algorithms
rely on core observations, notations and computations.
To make our presentation more modular and avoid repetition, we present these here as auxiliary functions and observations.
For the sake of completeness, we present the detailed algorithms and proofs
of these algorithms and observations in \cref{subsec:app_helper_functions},
while we refer to \cref{fig:helpers} for examples.

\input{figures/helpers}

\bparagraph{Happens-before computation}
%\scomment{It is possible that there exists no such event f for event e if there is no synchronization from t to e.tid.}
One common component in most of our algorithms is the computation of the $\hb$-timestamp $\HB_e : \E.tids \to \nats_{\geq 0}$ 
of each event $e$, declaratively defined as
\begin{align*}
%\label{eq:hb-timestamp}
\HB_e(t) = |\setpred{f}{f.\tid = t \land (f, e) \in \hb^?}|
\end{align*}
That is, $\HB_e(t)$ points to the latest event of thread $t$ that is $\hb$-ordered before (and including) $e$.
%\scomment{(Rephrasing without being specific for weaker accesses): The computation of all $\HB_e$ is easy for release-acquire or stronger accesses as the 
%$\rf$ edges imply synchronization, unlike the weaker accesses.} 
The computation of all $\HB_e$ is relatively straightforward under $\MOrel$/$\MOacq$ accesses,
but becomes more challenging when those are mixed with $\MOrlx$ accesses, as $\rf$ edges along $\MOrlx$ events do not induce a synchronization (see $\sw$ in \cref{subsec:executions}).
Nevertheless, we show that these timestamps can be computed in a \emph{streaming} fashion, 
in $O(\NumEvents \cdot \NumThreads)$ time.
In \cref{subsec:app_helper_functions} we present an algorithm \getHBTS{$\E$, $\po$, $\rf$} that returns
an $\E$-indexed array $\HB$ of $\hb$-timestamps, giving us:

\thmHBcomputation*

\bparagraph{Last write and last read functions}
Our consistency algorithms also use functions
$\glw$ and $\glr$ defined as follows.
Given a thread $t$, location $x$, and index $c \in \nats_{\geq 0}$, we define
\begin{align*}
\glw(t, x, c) = 
\begin{cases} \event & 
\begin{array}{l}\text{ if }  \event  \text{ is the last event $f$ such that, } f \in \locx{\W} \cup \locx{\U}, \\
		f.\tid = t \text{ and } |\setpred{g}{(g, f) \in \po^?}| \leq c \\
\end{array} \\
		\bot & \text{ if no such event exists} 
\end{cases}
\end{align*}
\begin{align*}
\glr(t, x, c) = 
\begin{cases} \event & 
\begin{array}{l}\text{ if }  \event  \text{ is the last event $f$ such that, } f \in \locx{\R} \cup \locx{\U}, \\
		f.\tid = t \text{ and } |\setpred{g}{(g, f) \in \po^?}| \leq c \\
\end{array} \\
		\bot & \text{ if no such event exists} 
\end{cases}
\end{align*}
In words, $\glw(t, x, c)$ returns the latest event $\wt(t,x)$ or $\U(t,x)$ that is $\po$-ordered before the $c$-th event of thread $t$ (similarly for $\glr(t, x, c)$).
Both functions can be computed by a simple scanning of $\expartial$ in $\po$-order, taking $O(\NumEvents\cdot \NumMemory)$ time in total.



\bparagraph{Top of, and position in  $\rf$-chain}
All memory models that we consider satisfy weak-atomicity,
i.e., no two RMW events can have the same writer.
This implies that all write and RMW events are arranged in disjoint \emph{$\rf$-chains},
where a chain is a sequence of events $\event_0, \event_1, \ldots, \event_{\ell}$ ($\ell \geq 0$), 
such that
(i)~$\event_0\in \W$ and $\event_1, \ldots, \event_\ell\in \U$, and
(ii)~$\rf(\event_{i})=\event_{i-1}$ for each $i\geq 1$.
\ucomment{Every RMW that reads from this chain also belongs to this \emph{maximal} chain}.
In words, we have a chain of events connected by $\rf$, starting with the top write event $e_0$, and (optionally) continuing with a sequence of RMW events.
Given an event $\event\in  (\WRMW)$, our consistency algorithms require access to the $\rf$-chain that $\event$ belongs to.
Specifically, for an event $\event$, the top of the chain $\TC[\event]$
is the unique event $f$ such that $(f, \event) \in \rf^*$ and $f.\op = \wt$.
The position $\PC[\event]$ of $e$ in its $\rf$-chain is the cardinality of the set
$\setpred{f}{(f, \event) \in \rf^+}$.
Both functions $\TC$ and $\PC$ can be computed in $O(\NumEvents)$ time.

\bparagraph{Conflicting triplets}
A \emph{conflicting triplet} (or just \emph{triplet}, for short) is a triplet of distinct events $(\event_1, \event_2, \event_3)$ such that
(i)~all events access the same location $x$,
(ii)~$\event_1, \event_3 \in (\locx{\W}\cup \locx{\U})$ and $\event_2\in (\locx{\R}\cup \locx{\U})$, and
(iii)~$\rf(\event_2)=\event_1$.

We start with a simple lemma that is instrumental throughout the paper.
It identifies certain $\mo$ orderings implied by the basic axioms of read-coherence, write-coherence and atomicity, and thus applies to all models except $\wramm$.

\begin{restatable}{lemma}{lemreadcoherenceatomicity}
\label{lem:read_coherence_atomicity}
Let $\ex = \tup{\E, \po, \rf, \mo}$ be an execution that satisfies read-coherence, write-coherence and atomicity.
Let $(\wt, \rd, \wt')$ be a triplet.
%and let $\wt^{\top}=\TC[\wt]$.
%If $(\wt', \rd)\in \hb$, or
%$(\wt', \rd)\in \rf;\hb^?$, then 
If $(\wt', \rd)\in \rf^?;\hb$ and 
$(\wt', \wt)\not \in \rf^+$, then
$(\wt', \TC[\wt])\in \mo$.
% \ucomment{Triplet not defined until this point. Similarly, $\TC$ is not defined until here.}
\end{restatable}
\ucomment{Add fig 6 here perhaps?}



%\begin{example}
%In \cref{fig:helpers} we compute some example helper functions on the given trace. We mark the access modes some events which are relevant for the computed helper functions. 
%On the trace the event pair $(e_3, e_6)$ is in $\sw$ relation. Hence, for event $e_7$, event $e_3$ is the latest $\hb$ predecessor in thread $T_1$, $\po$-predecessor event $e_6$ in $T_4$, and no $\hb$ predecessor in threads $T_2$ and $T-3$. 
%In thread $T_1$, given the third event $e_3$ and location $x$, the latest $\po$-predecessor write and read events are $e_1$ and $e_2$ respectively. Threads $T_2$ and $T_3$ has no access on location $x$. However, given thread $T_2$ and location $y$, 
%event $e_4$ itself is the latest write.
%On the trace, $e_3, e_4, e_5$ is the $\U$-chain and $e_3$ is the unique start event of the chain. Hence, we directly compute an $\mo$ relation from $e_3$ to $e_5$.
%\end{example}


==> models.tex <==
%!TEX root=./main.tex
\section{Formalization of Concurrency Semantics}\label{sec:models}

In this section we introduce the C/C++ concurrency semantics we consider in this work, along the RC20 model and its variants~\cite{Margalit:2021,Lahav:2022}.
As such, the exposition here is close to those works.

\bparagraph{Syntax} 
C/C++ defines shared memory concurrency model using different kinds of concurrency primitives. 
In addition to plain (or non-atomic) load and store accesses, C/C++ provides atomic accesses for load, store, atomic read-modify-write (RMW -- such as atomic increment), and fence operations.
We only consider atomic accesses here.
An atomic access is parameterized with a memory mode, among relaxed ($\MOrlx$), acquire ($\MOacq$), release ($\MOrel$), and acquire-release ($\MOacqrel$). 
%For the plain accesses we also consider non-atomic ($\MOna$) as a memory order.
Based on the operation and mode we categorize the accesses as follows:
\begin{align*}
acc ::= & \ \mathsf{read}_{o_r} \mid \mathsf{write}_{o_w} \mid \mathsf{RMW}_{o_u} \mid \mathsf{fence}_{o_f} \hfill \tag{accesses}
\\ o_r ::= & \ \MOrlx \mid \MOacq \tag{memory mode for read operation}
\\ o_w ::= & \ \MOrlx \mid \MOrel  \hfill \tag{memory mode for read operation}
\\ o_{u} ::= & \ \MOrlx \mid \MOacq \mid \MOrel \mid \MOacqrel  \tag{memory mode for RMW operation}
\\ o_{f} ::= & \ \MOacq \mid \MOrel \mid \MOacqrel  \tag{memory mode for fence operation}
\end{align*}
%\begin{align*}
%acc ::= & \ \mathsf{read}_{o_r} \mid \mathsf{write}_{o_w} \mid \mathsf{RMW}_{o_u} \mid \mathsf{fence}_{o_f} \hfill \tag{accesses}
%\\ o_r ::= & \ \MOna \mid \MOrlx \mid \MOacq \mid \MOsc  \tag{memory order for read operation}
%\\ o_w ::= & \ \MOna \mid \MOrlx \mid \MOrel \mid \MOsc \hfill \tag{memory order for read operation}
%\\ o_{u} ::= & \ \MOrlx \mid \MOacq \mid \MOrel \mid \MOacqrel \mid \MOsc \tag{memory order for RMW operation}
%\\ o_{f} ::= & \ \MOacq \mid \MOrel \mid \MOacqrel \mid \MOsc \tag{memory order for fence operation}
%\end{align*}
% \[
% \inarr{
% acc ::= \mathsf{read}_{(\MOna \mid \MOrlx \mid \MOacq \mid \MOsc)} \mid \mathsf{write}_{(\MOna \mid \MOrlx \mid \MOrel \mid \MOsc)} \mid \mathsf{RMW}_{(\MOrlx \mid \MOacq \mid \MOrel \mid \MOacqrel \mid \MOsc)} \mid \mathsf{fence}_{(\MOacq \mid \MOrel \mid \MOacqrel \mid \MOsc)}
% }
% \]
The memory modes are partially ordered on increasing strength of synchronization according to the lattice $\MOrlx \sqsubset \set{\MOacq,\MOrel} \sqsubset \MOacqrel$. 
An access is \emph{acquire} if its order is $\MOacq$ or stronger, that is, $\MOacq$, $\MOacqrel$, or $\MOsc$. Similarly an access is release if its order $\MOrel$ or stronger; that is, $\MOrel$, $\MOacqrel$, or $\MOsc$. 
Based on these syntactic primitives, a number of concurrency models have been proposed. 
These models are usually defined based on either axiomatic or operational semantics.
Here we discuss various axiomatic models, which are better suited for the consistency-checking problem we tackle in this work.


\input{executions}
\input{consistency_axioms}
\input{consistency_models}







==> related.tex <==
%!TEX root = ./main.tex

\section{Related Work}

Weak memory concurrency is widely explored in architectures \cite{Owens:2010,Alglave:2014,Pulte:2018,Alglave:2021}, compilers \cite{Chakraborty:2017,Podkopaev:2019}, and programming languages including C/C++ \cite{Adve:1990,Boehm:2008,Batty:2011,Vafeiadis:2015,Lahav:2017,Kang:2017,Chakraborty:2019,Bender:2019,Dang:2019,Margalit:2021,Lahav:2022}. 
% This is in introduction
In this paper we focus on the latest model C/C++ model RC20 and its variants \cite{Margalit:2021,Lahav:2022}. 
Side-by-side complexity theoretic analyses are studied for verification and testing under different consistency models.
%for developing testing and verification techniques. 
For instance, the verification problem is decidable for a number of consistency models including linearizability (NP-complete)\cite{Gibbons:1997}, TSO and PSO (non-primitive recursive) \cite{Atig:2010} as well as persistent-TSO (non-primitive recursive) \cite{Abdulla:2021}, coherence (NP-complete) \cite{Cantin:2005}, eventual consistency (EXPSPACE-hard) \cite{bouajjani:2014}. 
On the other hand the problem is undecidable for RMO \cite{Atig:2010}, Power \cite{Abdulla:netys:2020}, Quasi-linearizability \cite{wang:2015}, the relaxed fragment of PS2.0 \cite{Abdulla:2021b}, and RA \cite{Abdulla:2019} model. 
However, the reachability problem for WRA (equivalent to causal consistency \cite{bouajjani:2017}) and SRA, the weaker and stronger variants of RA, are decidable\cite{Lahav:2022}. 
%\citet{Furbach:2015} shows that the testing of the consistency models in \citet{Steinke-Nutt} are (mostly) NP-complete. 
%Related concurrency analyses problems with complexity results include state robustness against TSO (PSPACE-complete)\cite{Bouajjani:2011} and Power(PSPACE-complete) \cite{Derevenetc:2014}, atomicity checking (linear time) \cite{Mathur:2020}, race detection (NP-hard) \cite{Netzer:1990,Netzer:1992}, dynamic race prediction (W[1]-hard) \cite{Mathur:lics2020}, parameterized verification in TSO (PSPACE-complete) \cite{Abdulla:POPL:2020} and RA (PSPACE-complete) \cite{Shankaranarayanan:2022}.
%, execution-graph robustness against RA (decidable) \cite{Lahav:2019}, and observational robustness for RC20 (decidable) \cite{Lahav:2019}.

%A number of stateless model checking techniques are developed for SC and weaker models \cite{Abdulla:popl:2014,,Kokologiannakis:2018,Abdulla:2019b,Kokologiannakis:2022} that explore Mazurkiewicz traces \cite{Mazurkiewicz:1987}. 
%% We have discussed equivalent classes in detail in the paper already
%In contrary, the traces can be categorized in coarser-grain equivalence classes including read-from, read-value equivalence. 
%Based on these categorizations the analyses tools require to explore subset of executions for SC \cite{Abdulla:2019b, Chatterjee:2019,Agarwal:2021} as well as weaker models TSO and PSO \cite{Bui:2021}. 
%Our obtained results expands the horizon by testing C/C++ models for various equivalence classes. 

In recent years a number of weak memory concurrency agnostic tools are developed such as Herd toolsets \cite{Alglave:2014}, Nidhugg \cite{Abdulla:tacas:2015}, CDSChecker \cite{NorrisDemsky:2013}, GenMC \cite{Kokologiannakis:cav:2021} for verification, and \celeventester~\cite{Luo:2021}, tsan11 \cite{Lidbury:2017}, tsan11rec \cite{Lidbury:2019} for C11 testing. 
Our experiments on state-of-the-art tool \celeventester demonstrate the usability of the proposed algorithms towards developing scalable analysis tools in the future.


==> tab-experiments-2-old.tex <==
%!TEX root = main.tex

\begin{table}[H]
	\caption{
		Execution characteristics, and performance comparison. Column $1$ corresponds to the name of the benchmark. Columns $2$-$6$ denote the number of threads, locations, atomic read, write and RMW events. 
		Columns $7$-$11$ and $12$-$16$ denote the saturation times of \celeventester and \cref{algo:ra-rf-on-the-fly} for read events, write events, RMW events, propagation and total time.
		Column 17 denotes the overall speedup.
		\label{tab:expr-results-2}
	}
	\setlength\tabcolsep{0.8pt}
	\renewcommand{\arraystretch}{0.9}
	\centering
	%\scalebox{1}{
{\small
		\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c||c|c|c|c|c|c|}
			\hline
			1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 14 & 15 & 16 & 17 \\
			\hline
			\multirow{2}{*}{\textbf{Benchmark}}& 
			\multirow{2}{*}{$\mathcal{T}$} &
			\multirow{2}{*}{$\mathcal{L}$} &
			\multirow{2}{*}{$\mathcal{R}$}
			&
			\multirow{2}{*}{$\mathcal{W}$}
			& \multirow{2}{*}{$\mathcal{U}$}
			&
			\multicolumn{5}{c||}{ {\rule{0pt}{1em} \celeventester} } & 
			
			\multicolumn{5}{c|}{ {\cref{algo:ra-rf-on-the-fly}} } 
			& \multirow{2}{*}{Speed-}
			 \\
			
			\cline{7-11}
			\cline{12-16}
			
				& & & & & & \rule{0pt}{1em} $\rd$ & $\wt$ & $\ud$ & $\mathsf{P}$ & Total & $\rd$ & $\wt$ & $\ud$ & $\mathsf{P}$ & Total & up
		\\
			\hline
\rule{0pt}{1em} 
control-flow & 25  & 3  & 28K  & 24K  & 0  & 0.01 & 4.2  & 0.0 & 0.01 & 4.2  & 0.01 & 0.01 & 0.0 & 0.01 & 0.04 & 99.38 \\
sigma & 10  & 9  & 18K  & 18K  & 0  & 0.0 & 2.4  & 0.0 & 0.0 & 2.4  & 0.01 & 0.01 & 0.0 & 0.0 & 0.03 & 93.34 \\
dq & 4  & 2  & 471K  & 114K  & 14K  & 7.5  & 14.5  & 0.01 & 0.09 & 22.1  & 0.3  & 0.03 & 0.0 & 0.09 & 0.5  & 46.78 \\
iris-1 & 12  & 45  & 502K  & 500K  & 56K  & 0.5  & 27.6  & 0.04 & 0.2  & 28.4  & 1.2  & 0.2  & 0.01 & 0.1  & 1.8  & 16.25 \\
seqlock & 17  & 20  & 361K  & 117K  & 0  & 5.4  & 8.8  & 0.0 & 0.2  & 14.4  & 1.3  & 0.06 & 0.0 & 0.1 & 1.4  & 10.38 \\
exp-bug & 4  & 2  & 234K  & 2M  & 0  & 0.1 & 1.5  & 0.0 & 0.05 & 1.6  & 0.1  & 0.5  & 0.0 & 0.04 & 0.7  & 2.35 \\
CLDQ & 5  & 2  & 6M  & 1M  & 500K  & 5.1  & 5.5  & 0.4  & 1.4  & 12.4  & 2.9  & 0.4  & 0.2  & 1.1  & 5.4  & 2.3 \\
linuxrwlocks & 6  & 10  & 1M  & 10  & 6M  & 2.8  & 2.8  & 3.4  & 1.9  & 10.9  & 2.2  & 1.2  & 1.1  & 1.2  & 5.9  & 1.84 \\
mabain & 6  & 18  & 527  & 780  & 5M  & 1.4  & 2.0  & 2.8  & 1.1  & 7.3  & 1.3  & 1.0  & 0.9  & 0.9  & 4.0  & 1.82 \\
iris-2 & 3  & 12  & 6M  & 4M  & 2M  & 2.8  & 4.6  & 1.1  & 1.5  & 9.9  & 2.4  & 1.3  & 0.4  & 1.4  & 5.7  & 1.72 \\
mcs-lock & 11  & 30  & 5M  & 4M  & 2M  & 8.3  & 6.4  & 1.1  & 1.9  & 17.8  & 7.9  & 1.4  & 0.4  & 1.1  & 12.2  & 1.45 \\
lamport & 3  & 5  & 3M  & 3M  & 0  & 0.9  & 1.9  & 0.0 & 0.5  & 3.4  & 1.1  & 0.7  & 0.0 & 0.4  & 2.5  & 1.36 \\
peterson & 3  & 4  & 3M  & 2M  & 0  & 0.8  & 1.5  & 0.0 & 0.6  & 2.9  & 1.0  & 0.5  & 0.0 & 0.5  & 2.2  & 1.29 \\
spsc & 3  & 699  & 5M  & 4M  & 851K  & 2.0  & 2.8  & 0.5  & 1.2  & 6.4  & 2.1  & 1.1  & 0.2  & 1.1  & 5.0  & 1.28 \\
dekker & 3  & 3  & 9M  & 7M  & 0  & 3.1  & 4.5  & 0.0 & 1.6  & 9.2  & 3.6  & 1.6  & 0.0 & 1.5  & 7.2  & 1.27 \\
twalock & 11  & 4K  & 3M  & 500K  & 1M  & 5.4  & 1.6  & 0.7  & 1.3  & 8.9  & 4.6  & 0.4  & 0.2  & 0.8  & 7.0  & 1.26 \\
mutex & 11  & 11  & 7M  & 1M  & 6M  & 8.1  & 4.4  & 4.8  & 3.5  & 20.9  & 8.6  & 1.8  & 2.0  & 2.7  & 16.8  & 1.24 \\
gdax & 5  & 46K  & 4M  & 5M  & 2M  & 1.4  & 3.2  & 1.3  & 1.1  & 7.0  & 1.8  & 1.6  & 0.5  & 1.1  & 5.7  & 1.23 \\
spinlock & 11  & 10  & 3M  & 1M  & 1M  & 3.1  & 2.1  & 0.7  & 1.1  & 7.0  & 3.7  & 0.5  & 0.3  & 0.7  & 5.9  & 1.18 \\
ticketlock & 6  & 20  & 9M  & 2M  & 2M  & 7.8  & 3.7  & 1.5  & 2.7  & 15.7  & 8.1  & 1.2  & 0.5  & 2.0  & 13.2  & 1.18 \\
ttaslock & 11  & 10  & 3M  & 1M  & 1M  & 3.3  & 2.4  & 1.0  & 1.1  & 7.8  & 4.3  & 0.6  & 0.3  & 0.8  & 6.6  & 1.18 \\
fib-bench & 3  & 2  & 4M  & 2M  & 0  & 1.3  & 1.2  & 0.0 & 0.8  & 3.3  & 1.4  & 0.4  & 0.0 & 0.7  & 2.8  & 1.18 \\
qu & 10  & 29  & 912K  & 336K  & 0  & 0.9  & 0.4  & 0.0 & 0.2  & 1.6  & 0.9  & 0.08 & 0.0 & 0.2  & 1.3  & 1.18 \\
treiber & 6  & 11  & 753K  & 158K  & 100K  & 0.6  & 0.2  & 0.1 & 0.2  & 1.1  & 0.6  & 0.06 & 0.05 & 0.1  & 1.0  & 1.12 \\
silo & 4  & 4K  & 5M  & 3M  & 756K  & 2.1  & 1.9  & 0.4  & 1.0  & 5.3  & 2.2  & 0.8  & 0.1  & 0.9  & 4.8  & 1.1 \\
barrier & 5  & 20  & 6M  & 300K  & 2M  & 4.4  & 0.9  & 0.9  & 1.5  & 7.8  & 4.5  & 0.4  & 0.3  & 1.3  & 7.4  & 1.04 \\
mpmc & 10  & 3  & 8M  & 3  & 1M  & 8.6  & 1.1  & 1.1  & 2.0  & 12.9  & 8.0  & 0.3  & 0.5  & 1.7  & 12.5  & 1.03 \\
indexer & 17  & 128  & 2M  & 256  & 0  & 1.2  & 0.0 & 0.0 & 0.3  & 1.6  & 0.8  & 0.0 & 0.0 & 0.4  & 1.5  & 1.03 \\
buf-ring & 9  & 12  & 4M  & 434K  & 289K  & 4.7  & 0.9  & 0.3  & 1.1  & 7.0  & 4.6  & 0.2  & 0.2  & 0.8  & 6.8  & 1.02 \\
ms-queue & 11  & 13  & 4M  & 100K  & 300K  & 6.2  & 0.6  & 0.3  & 1.1  & 8.2  & 5.8  & 0.1  & 0.1  & 0.8  & 8.2  & 0.99 \\
gcd & 3  & 2  & 4M  & 300K  & 0  & 1.3  & 0.2  & 0.0 & 0.7  & 2.2  & 1.5  & 0.07 & 0.0 & 0.7  & 2.5  & 0.89 \\
szymanski & 3  & 3  & 4M  & 17K  & 0  & 1.2  & 0.01 & 0.0 & 0.6  & 1.8  & 1.4  & 0.0 & 0.0 & 0.7  & 2.3  & 0.81 \\
JSBench & 13  & 3K  & 302K  & 13K  & 27K  & 0.1 & 0.02 & 0.02 & 0.06 & 0.2  & 0.1  & 0.01 & 0.01 & 0.06 & 0.3  & 0.77 \\
\hline\hline\textbf{Total} & \textbf{312} & \textbf{58K} & \textbf{115M} & \textbf{47M} & \textbf{35M} & \textbf{110.8} & \textbf{118.9} & \textbf{22.5} & \textbf{34.5} & \textbf{286.6} & \textbf{95.8} & \textbf{18.9} & \textbf{8.0} & \textbf{27.6} & \textbf{171.1} & \textbf{}\\
			\hline
		\end{tabular}
}  
	%}
\end{table}


==> tab-experiments-3.tex <==
%!TEX root = main.tex

\begin{table}
	\caption{
		Execution characteristics, and performance comparison. Column $1$ corresponds to the name of the benchmark. Columns $2$-$6$ denote the number of threads, locations, atomic read, write and RMW events. 
		Columns $7$-$11$ and $12$-$16$ denote the saturation times of \celeventester and \cref{algo:ra-rf-on-the-fly} for read events, write events, RMW events, propagation and total time.
		Column 17 denotes the overall speedup.
		\label{tab:expr-results-3}
	}
	\setlength\tabcolsep{0.8pt}
	\renewcommand{\arraystretch}{0.9}
	\centering
	%\scalebox{1}{
{\small
		\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c||c|c|c|c|c|c|}
			\hline
			1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 14 & 15 & 16 & 17 \\
			\hline
			\multirow{2}{*}{\textbf{Benchmark}}& 
			\multirow{2}{*}{$\mathcal{T}$} &
			\multirow{2}{*}{$\mathcal{L}$} &
			\multirow{2}{*}{$\mathcal{R}$}
			&
			\multirow{2}{*}{$\mathcal{W}$}
			& \multirow{2}{*}{$\mathcal{U}$}
			&
			\multicolumn{5}{c||}{ {\rule{0pt}{1em} \celeventester} } & 
			
			\multicolumn{5}{c|}{ {\cref{algo:ra-rf-on-the-fly}} } 
			& \multirow{2}{*}{Speed-}
			 \\
			
			\cline{7-11}
			\cline{12-16}
			
				& & & & & & \rule{0pt}{1em} $\rd$ & $\wt$ & $\ud$ & $\mathsf{P}$ & Total & $\rd$ & $\wt$ & $\ud$ & $\mathsf{P}$ & Total & up
		\\
			\hline
\rule{0pt}{1em} 
control-flow & 25  & 3  & 28K  & 24K  & 0  & 0.01 & 4.2  & 0.0 & 0.01 & 4.2  & 0.01 & 0.01 & 0.0 & 0.01 & 0.04 & 99.38 \\
sigma & 10  & 9  & 18K  & 18K  & 0  & 0.0 & 2.4  & 0.0 & 0.0 & 2.4  & 0.01 & 0.01 & 0.0 & 0.0 & 0.03 & 93.34 \\
dq & 4  & 2  & 471K  & 114K  & 14K  & 7.5  & 14.5  & 0.01 & 0.09 & 22.1  & 0.3  & 0.03 & 0.0 & 0.09 & 0.5  & 46.78 \\
iris-1 & 12  & 45  & 502K  & 500K  & 56K  & 0.5  & 27.6  & 0.04 & 0.2  & 28.4  & 1.2  & 0.2  & 0.01 & 0.1  & 1.8  & 16.25 \\
seqlock & 17  & 20  & 361K  & 117K  & 0  & 5.4  & 8.8  & 0.0 & 0.2  & 14.4  & 1.3  & 0.06 & 0.0 & 0.1 & 1.4  & 10.38 \\
mabain & 6  & 18  & 527  & 780  & 5M  & 1.4  & 2.0  & 2.8  & 1.1  & 7.3  & 1.3  & 1.0  & 0.9  & 0.9  & 4.0  & 1.82 \\
iris-2 & 3  & 12  & 6M  & 4M  & 2M  & 2.8  & 4.6  & 1.1  & 1.5  & 9.9  & 2.4  & 1.3  & 0.4  & 1.4  & 5.7  & 1.72 \\
silo & 4  & 4K  & 5M  & 3M  & 756K  & 2.1  & 1.9  & 0.4  & 1.0  & 5.3  & 2.2  & 0.8  & 0.1  & 0.9  & 4.8  & 1.1 \\
% barrier & 5  & 20  & 6M  & 300K  & 2M  & 4.4  & 0.9  & 0.9  & 1.5  & 7.8  & 4.5  & 0.4  & 0.3  & 1.3  & 7.4  & 1.04 \\
% gcd & 3  & 2  & 4M  & 300K  & 0  & 1.3  & 0.2  & 0.0 & 0.7  & 2.2  & 1.5  & 0.07 & 0.0 & 0.7  & 2.5  & 0.89 \\
% szymanski & 3  & 3  & 4M  & 17K  & 0  & 1.2  & 0.01 & 0.0 & 0.6  & 1.8  & 1.4  & 0.0 & 0.0 & 0.7  & 2.3  & 0.81 \\
%JSBench & 13  & 3K  & 302K  & 13K  & 27K  & 0.1 & 0.02 & 0.02 & 0.06 & 0.2  & 0.1  & 0.01 & 0.01 & 0.06 & 0.3  & 0.77 \\
\hline\hline\textbf{Total} & \textbf{312} & \textbf{58K} & \textbf{115M} & \textbf{47M} & \textbf{35M} & \textbf{110.8} & \textbf{118.9} & \textbf{22.5} & \textbf{34.5} & \textbf{286.6} & \textbf{95.8} & \textbf{18.9} & \textbf{8.0} & \textbf{27.6} & \textbf{171.1} & \textbf{}\\
			\hline
		\end{tabular}
}  
	%}
\end{table}


==> tab_experiments.tex <==
%!TEX root = main.tex

\begin{table}[H]
	\caption{
		Performance comparison of \celeventester and \cref{algo:ra-rf-on-the-fly} in the settings \expsetone and \expsettwo.
		\label{tab:expr-results}
	}
	\setlength\tabcolsep{3pt}
	\renewcommand{\arraystretch}{1}
	\centering
	%\scalebox{1}{
		\begin{tabular}{|c|c|c|c||c|c|c|}
			\hline
			1 & 2 & 3 & 4 & 5 & 6 & 7 \\
			\hline
			\multirow{2}{*}{\textbf{Benchmark}}& 
			\multicolumn{3}{c||}{ {\rule{0pt}{1em}  \expsettwo (Independent Executions)} } & 
			
			\multicolumn{3}{c|}{ { \expsetone (Same Execution)} } 
			 \\
			
			\cline{2-4}
			\cline{5-7}
			
			& \rule{0pt}{1em} \celeventester & \cref{algo:ra-rf-on-the-fly} & Speedup & \celeventester & \cref{algo:ra-rf-on-the-fly}  
			& Speedup
		\\
			\hline
dq & 21.68 (0.30) & 0.83 (0.02) & 26.02  & 22.08 (0.37) & 0.47 (0.01) & 46.78 \\
iris-1 & 47.08 (0.77) & 24.11 (0.25) & 1.95  & 28.38 (0.33) & 1.75 (0.04) & 16.25 \\
seqlock & 14.42 (0.20) & 1.39 (0.04) & 10.35  & 14.39 (0.16) & 1.39 (0.03) & 10.38 \\
CLDQ & 23.40 (5.20) & 16.98 (0.30) & 1.37  & 12.39 (5.65) & 5.38 (0.05) & 2.3 \\
linuxrwlocks & 17.61 (0.17) & 13.46 (0.13) & 1.3  & 10.93 (0.19) & 5.92 (0.12) & 1.84 \\
mabain & 14.56 (0.14) & 11.84 (0.21) & 1.23  & 7.30 (0.17) & 4.00 (0.09) & 1.82 \\
iris-2 & 19.00 (0.43) & 14.86 (0.16) & 1.27  & 9.88 (0.19) & 5.74 (0.11) & 1.72 \\
mcs-lock & 26.63 (0.46) & 21.48 (0.25) & 1.24  & 17.77 (0.36) & 12.20 (0.37) & 1.45 \\
spsc-queue & 15.06 (0.37) & 14.03 (0.20) & 1.07  & 6.44 (0.12) & 4.99 (0.10) & 1.28 \\
dekker-fences & 21.04 (0.25) & 19.23 (0.33) & 1.09  & 9.18 (0.15) & 7.23 (0.14) & 1.27 \\
twalock & 13.01 (0.25) & 10.25 (0.40) & 1.26  & 8.94 (0.22) & 7.05 (0.17) & 1.26 \\
mutex & 31.88 (0.63) & 28.95 (0.65) & 1.1  & 20.92 (0.38) & 16.83 (0.35) & 1.24 \\
spinlock & 10.21 (0.10) & 9.28 (0.12) & 1.09  & 7.00 (0.12) & 5.94 (0.10) & 1.18 \\
ticketlock & 21.61 (0.26) & 19.44 (0.32) & 1.11  & 15.70 (0.31) & 13.21 (0.24) & 1.18 \\
ttaslock & 11.04 (0.20) & 9.84 (0.14) & 1.12  & 7.80 (0.14) & 6.60 (0.12) & 1.18 \\
treiber-stack & 1.50 (0.02) & 1.43 (0.04) & 1.05  & 1.13 (0.02) & 1.00 (0.02) & 1.12 \\
silo (*) & 29K (202.47) & 30K (111.11) & 1.02  & 5.29 (0.01) & 4.77 (0.01) & 1.1 \\
barrier & 14.24 (0.52) & 13.60 (0.15) & 1.04  & 7.75 (0.09) & 7.44 (0.09) & 1.04 \\
mpmc-queue & 21.49 (0.34) & 21.54 (0.38) & 0.99  & 12.89 (0.13) & 12.47 (0.13) & 1.03 \\
buf-ring & 9.20 (0.19) & 9.03 (0.16) & 1.01  & 6.96 (0.06) & 6.78 (0.05) & 1.02 \\
ms-queue & 10.70 (0.20) & 10.90 (0.15) & 0.98  & 8.19 (0.24) & 8.22 (0.22) & 0.99 \\
			\hline
			\hline
			\textbf{Average} & \textbf{} & & \textbf{2.88} & \textbf{} &  & \textbf{4.82}
			\\
			\hline
		\end{tabular}
	%}
\end{table}


==> tab_intro.tex <==
%\begin{table}
%\renewcommand{\arraystretch}{1.2}
%\aboverulesep=0ex
%\belowrulesep=0ex
%\caption{
%\label{tab:intro}
%The complexity of consistency problems for various concurrent memory models, on an input of size $\NumEvents$ over $\NumThreads$ threads and $\NumMemory$ variables.
%}
%\begin{tabular}{|c||c|c|c|}
%\hline
%& RF & RV+MO & RV \\
%\midrule[1pt]
%SRA & \makecell{$\NP$-hard\\$O(\NumThreads\cdot \NumEvents^{\NumThreads})$}  & $O(\NumEvents\cdot(\NumThreads + \NumMemory))$ for single-writer & $\NP$ \\
%\hdashline
%SRA w/o RMWs & $O(\NumEvents\cdot(\NumThreads + \NumMemory))$ & $\NP$-hard& \makecell{$\NP$-hard for $k=3$\\ $\NP$-hard for $d=1$}\\
%\midrule
%WRA & $O(\NumEvents\cdot(\NumThreads + \NumMemory))$ & $O(\NumEvents\cdot(\NumThreads + \NumMemory))$ for single-writer & $\NP$ \\
%\hdashline
%WRA w/o RMWs & -  & $\NP$-hard  & \makecell{$\NP$-hard for $k=4$\\ $\NP$-hard for $d=1$}\\
%\midrule
%RC20 & $O(\NumEvents\cdot(\NumThreads + \NumMemory))$ & $O(\NumEvents\cdot(\NumThreads + \NumMemory))$ for single-writer & $\NP$ \\
%\hdashline
%RA w/o RMWs & - & $\NP$-hard & \makecell{$\NP$-hard for $k=3$\\ $\NP$-hard for $d=1$}\\
%\midrule
%Relaxed & $O(\NumEvents)$ & \makecell{$O(\NumEvents\cdot\NumThreads)$ for single-writer} & $\NP$ \\
%\hdashline
%Relaxed w/o RMWs & - & & \makecell{$\NP$-hard for $k=3$ \Andreas{revisit}\\ $\NP$-hard for $d=1$}\\
%\bottomrule
%\end{tabular}
%\end{table}


\begin{table}
\renewcommand{\arraystretch}{1.2}
\aboverulesep=0ex
\belowrulesep=0ex
\caption{
\label{tab:intro}
The complexity of consistency problems for various concurrent memory models, on an input of size $\NumEvents$ over $\NumThreads$ threads and $\NumMemory$ variables.
All hardness results except RF consistency under SRA hold even without the presence of RMWs.
$\dagger$:~Subsumed by the same result for $\rcmm$.
$\ddagger$~Subsumed by the same result for $\ramm$.
}
\begin{tabular}{|c||c|c|c|}
\hline
& RF & RV+MO & RV \\
\midrule[1pt]
$\sramm$ & \makecell{$\NP$-hard  \\$O(\NumThreads\cdot \NumEvents^{\NumThreads})$  \\$O(\NumEvents\cdot(\NumThreads + \NumMemory))$ w/o RMWs}  & \makecell{$O(\NumEvents\cdot(\NumThreads + \NumMemory))$ for unique writers  \\ $\NP$-hard} & \makecell{$\NP$-hard for $k=3$  \\ $\NP$-hard for $d=1$} \\
%\hdashline
%SRA w/o RMWs & $O(\NumEvents\cdot(\NumThreads + \NumMemory))$ & \makecell{$O(\NumEvents\cdot(\NumThreads + \NumMemory))$\\ $\NP$-hard}& \makecell{$\NP$-hard for $k=3$\\ $\NP$-hard for $d=1$}\\
\midrule
$\ramm$ & $O(\NumEvents\cdot(\NumThreads + \NumMemory))^{\dagger}$ & \makecell{$O(\NumEvents\cdot(\NumThreads + \NumMemory))$ for unique writers \\ $\NP$-hard} & \makecell{$\NP$-hard for $k=3$ \\ $\NP$-hard for $d=1$} \\
\midrule
$\wramm$ & $O(\NumEvents\cdot(\NumThreads + \NumMemory))$ & \makecell{$O(\NumEvents\cdot(\NumThreads + \NumMemory))$ for unique writers  \\ $\NP$-hard}  & \makecell{$\NP$-hard for $k=4$  \\  $\NP$-hard for $d=1$} \\
%\hdashline
%WRA w/o RMWs & $O(\NumEvents\cdot(\NumThreads + \NumMemory))^{\ddagger}$  & $\NP$-hard  & \makecell{$\NP$-hard for $k=4$\\ $\NP$-hard for $d=1$}\\
%\hdashline
%RA w/o RMWs & $O(\NumEvents\cdot(\NumThreads + \NumMemory))^{\ddagger}$ & $\NP$-hard & \makecell{$\NP$-hard for $k=3$\\ $\NP$-hard for $d=1$}\\
\midrule
$\rlxmm$ & $O(\NumEvents)$ & \makecell{$O(\NumEvents)$ for unique writers  \\ $\NP$-hard} & \makecell{$\NP$-hard for $k=7$  \\ $\NP$-hard for $d=1$} \\
%\hdashline
%Relaxed w/o RMWs & $O(\NumEvents\cdot\NumThreads)^{\ddagger}$ & & \makecell{$\NP$-hard for $k=3$\\ $\NP$-hard for $d=1$}\\
\midrule
$\rcmm$ & $O(\NumEvents\cdot(\NumThreads + \NumMemory))$ & \makecell{$\NP$-hard for unique writers} & \makecell{$\NP$-hard for $k=3^{\ddagger}$ \\ $\NP$-hard for $d=1^{\ddagger}$} \\
%\hdashline
%RA w/o RMWs & $O(\NumEvents\cdot(\NumThreads + \NumMemory))^{\ddagger}$ & $\NP$-hard & \makecell{$\NP$-hard for $k=3$\\ $\NP$-hard for $d=1$}\\
\bottomrule
\end{tabular}
\end{table}
